A search for weakly decaying b-flavored pentaquarks

Investigations of the existence of pentaquark states containing a single $b$ (anti)quark decaying weakly into four specific final states J/$\psi K^+\pi^- p$, J/$\psi K^- \pi^- p$, J/$\psi K^- \pi^+ p$, and $J/\psi \phi (1020) p$ are reported. The data sample corresponds to an integrated luminosity of 3.0/fb in 7 and 8 TeV pp collisions acquired with the LHCb detector. Signals are not observed and upper limits are set on the product of the production cross section times branching fraction with respect to that of the $\Lambda_b$.

==> LHCb_Authorship_flat_13-Oct-2017.tex <==
\centerline{\large\bf LHCb collaboration}
\begin{flushleft}
\small
R.~Aaij$^{40}$,
B.~Adeva$^{39}$,
M.~Adinolfi$^{48}$,
Z.~Ajaltouni$^{5}$,
S.~Akar$^{59}$,
J.~Albrecht$^{10}$,
F.~Alessio$^{40}$,
M.~Alexander$^{53}$,
A.~Alfonso~Albero$^{38}$,
S.~Ali$^{43}$,
G.~Alkhazov$^{31}$,
P.~Alvarez~Cartelle$^{55}$,
A.A.~Alves~Jr$^{59}$,
S.~Amato$^{2}$,
S.~Amerio$^{23}$,
Y.~Amhis$^{7}$,
L.~An$^{3}$,
L.~Anderlini$^{18}$,
G.~Andreassi$^{41}$,
M.~Andreotti$^{17,g}$,
J.E.~Andrews$^{60}$,
R.B.~Appleby$^{56}$,
F.~Archilli$^{43}$,
P.~d'Argent$^{12}$,
J.~Arnau~Romeu$^{6}$,
A.~Artamonov$^{37}$,
M.~Artuso$^{61}$,
E.~Aslanides$^{6}$,
M.~Atzeni$^{42}$,
G.~Auriemma$^{26}$,
M.~Baalouch$^{5}$,
I.~Babuschkin$^{56}$,
S.~Bachmann$^{12}$,
J.J.~Back$^{50}$,
A.~Badalov$^{38,m}$,
C.~Baesso$^{62}$,
S.~Baker$^{55}$,
V.~Balagura$^{7,b}$,
W.~Baldini$^{17}$,
A.~Baranov$^{35}$,
R.J.~Barlow$^{56}$,
C.~Barschel$^{40}$,
S.~Barsuk$^{7}$,
W.~Barter$^{56}$,
F.~Baryshnikov$^{32}$,
V.~Batozskaya$^{29}$,
V.~Battista$^{41}$,
A.~Bay$^{41}$,
L.~Beaucourt$^{4}$,
J.~Beddow$^{53}$,
F.~Bedeschi$^{24}$,
I.~Bediaga$^{1}$,
A.~Beiter$^{61}$,
L.J.~Bel$^{43}$,
N.~Beliy$^{63}$,
V.~Bellee$^{41}$,
N.~Belloli$^{21,i}$,
K.~Belous$^{37}$,
I.~Belyaev$^{32,40}$,
E.~Ben-Haim$^{8}$,
G.~Bencivenni$^{19}$,
S.~Benson$^{43}$,
S.~Beranek$^{9}$,
A.~Berezhnoy$^{33}$,
R.~Bernet$^{42}$,
D.~Berninghoff$^{12}$,
E.~Bertholet$^{8}$,
A.~Bertolin$^{23}$,
C.~Betancourt$^{42}$,
F.~Betti$^{15}$,
M.O.~Bettler$^{40}$,
M.~van~Beuzekom$^{43}$,
Ia.~Bezshyiko$^{42}$,
S.~Bifani$^{47}$,
P.~Billoir$^{8}$,
A.~Birnkraut$^{10}$,
A.~Bizzeti$^{18,u}$,
M.~Bj{\o}rn$^{57}$,
T.~Blake$^{50}$,
F.~Blanc$^{41}$,
S.~Blusk$^{61}$,
V.~Bocci$^{26}$,
T.~Boettcher$^{58}$,
A.~Bondar$^{36,w}$,
N.~Bondar$^{31}$,
I.~Bordyuzhin$^{32}$,
S.~Borghi$^{56,40}$,
M.~Borisyak$^{35}$,
M.~Borsato$^{39}$,
F.~Bossu$^{7}$,
M.~Boubdir$^{9}$,
T.J.V.~Bowcock$^{54}$,
E.~Bowen$^{42}$,
C.~Bozzi$^{17,40}$,
S.~Braun$^{12}$,
J.~Brodzicka$^{27}$,
D.~Brundu$^{16}$,
E.~Buchanan$^{48}$,
C.~Burr$^{56}$,
A.~Bursche$^{16,f}$,
J.~Buytaert$^{40}$,
W.~Byczynski$^{40}$,
S.~Cadeddu$^{16}$,
H.~Cai$^{64}$,
R.~Calabrese$^{17,g}$,
R.~Calladine$^{47}$,
M.~Calvi$^{21,i}$,
M.~Calvo~Gomez$^{38,m}$,
A.~Camboni$^{38,m}$,
P.~Campana$^{19}$,
D.H.~Campora~Perez$^{40}$,
L.~Capriotti$^{56}$,
A.~Carbone$^{15,e}$,
G.~Carboni$^{25,j}$,
R.~Cardinale$^{20,h}$,
A.~Cardini$^{16}$,
P.~Carniti$^{21,i}$,
L.~Carson$^{52}$,
K.~Carvalho~Akiba$^{2}$,
G.~Casse$^{54}$,
L.~Cassina$^{21}$,
M.~Cattaneo$^{40}$,
G.~Cavallero$^{20,40,h}$,
R.~Cenci$^{24,t}$,
D.~Chamont$^{7}$,
M.G.~Chapman$^{48}$,
M.~Charles$^{8}$,
Ph.~Charpentier$^{40}$,
G.~Chatzikonstantinidis$^{47}$,
M.~Chefdeville$^{4}$,
S.~Chen$^{16}$,
S.F.~Cheung$^{57}$,
S.-G.~Chitic$^{40}$,
V.~Chobanova$^{39}$,
M.~Chrzaszcz$^{42}$,
A.~Chubykin$^{31}$,
P.~Ciambrone$^{19}$,
X.~Cid~Vidal$^{39}$,
G.~Ciezarek$^{40}$,
P.E.L.~Clarke$^{52}$,
M.~Clemencic$^{40}$,
H.V.~Cliff$^{49}$,
J.~Closier$^{40}$,
V.~Coco$^{40}$,
J.~Cogan$^{6}$,
E.~Cogneras$^{5}$,
V.~Cogoni$^{16,f}$,
L.~Cojocariu$^{30}$,
P.~Collins$^{40}$,
T.~Colombo$^{40}$,
A.~Comerma-Montells$^{12}$,
A.~Contu$^{16}$,
G.~Coombs$^{40}$,
S.~Coquereau$^{38}$,
G.~Corti$^{40}$,
M.~Corvo$^{17,g}$,
C.M.~Costa~Sobral$^{50}$,
B.~Couturier$^{40}$,
G.A.~Cowan$^{52}$,
D.C.~Craik$^{58}$,
A.~Crocombe$^{50}$,
M.~Cruz~Torres$^{1}$,
R.~Currie$^{52}$,
C.~D'Ambrosio$^{40}$,
F.~Da~Cunha~Marinho$^{2}$,
C.L.~Da~Silva$^{73}$,
E.~Dall'Occo$^{43}$,
J.~Dalseno$^{48}$,
A.~Davis$^{3}$,
O.~De~Aguiar~Francisco$^{40}$,
K.~De~Bruyn$^{40}$,
S.~De~Capua$^{56}$,
M.~De~Cian$^{12}$,
J.M.~De~Miranda$^{1}$,
L.~De~Paula$^{2}$,
M.~De~Serio$^{14,d}$,
P.~De~Simone$^{19}$,
C.T.~Dean$^{53}$,
D.~Decamp$^{4}$,
L.~Del~Buono$^{8}$,
H.-P.~Dembinski$^{11}$,
M.~Demmer$^{10}$,
A.~Dendek$^{28}$,
D.~Derkach$^{35}$,
O.~Deschamps$^{5}$,
F.~Dettori$^{54}$,
B.~Dey$^{65}$,
A.~Di~Canto$^{40}$,
P.~Di~Nezza$^{19}$,
H.~Dijkstra$^{40}$,
F.~Dordei$^{40}$,
M.~Dorigo$^{40}$,
A.~Dosil~Su{\'a}rez$^{39}$,
L.~Douglas$^{53}$,
A.~Dovbnya$^{45}$,
K.~Dreimanis$^{54}$,
L.~Dufour$^{43}$,
G.~Dujany$^{8}$,
P.~Durante$^{40}$,
J.M.~Durham$^{73}$,
D.~Dutta$^{56}$,
R.~Dzhelyadin$^{37}$,
M.~Dziewiecki$^{12}$,
A.~Dziurda$^{40}$,
A.~Dzyuba$^{31}$,
S.~Easo$^{51}$,
M.~Ebert$^{52}$,
U.~Egede$^{55}$,
V.~Egorychev$^{32}$,
S.~Eidelman$^{36,w}$,
S.~Eisenhardt$^{52}$,
U.~Eitschberger$^{10}$,
R.~Ekelhof$^{10}$,
L.~Eklund$^{53}$,
S.~Ely$^{61}$,
S.~Esen$^{12}$,
H.M.~Evans$^{49}$,
T.~Evans$^{57}$,
A.~Falabella$^{15}$,
N.~Farley$^{47}$,
S.~Farry$^{54}$,
D.~Fazzini$^{21,i}$,
L.~Federici$^{25}$,
D.~Ferguson$^{52}$,
G.~Fernandez$^{38}$,
P.~Fernandez~Declara$^{40}$,
A.~Fernandez~Prieto$^{39}$,
F.~Ferrari$^{15}$,
L.~Ferreira~Lopes$^{41}$,
F.~Ferreira~Rodrigues$^{2}$,
M.~Ferro-Luzzi$^{40}$,
S.~Filippov$^{34}$,
R.A.~Fini$^{14}$,
M.~Fiorini$^{17,g}$,
M.~Firlej$^{28}$,
C.~Fitzpatrick$^{41}$,
T.~Fiutowski$^{28}$,
F.~Fleuret$^{7,b}$,
M.~Fontana$^{16,40}$,
F.~Fontanelli$^{20,h}$,
R.~Forty$^{40}$,
V.~Franco~Lima$^{54}$,
M.~Frank$^{40}$,
C.~Frei$^{40}$,
J.~Fu$^{22,q}$,
W.~Funk$^{40}$,
E.~Furfaro$^{25,j}$,
C.~F{\"a}rber$^{40}$,
E.~Gabriel$^{52}$,
A.~Gallas~Torreira$^{39}$,
D.~Galli$^{15,e}$,
S.~Gallorini$^{23}$,
S.~Gambetta$^{52}$,
M.~Gandelman$^{2}$,
P.~Gandini$^{22}$,
Y.~Gao$^{3}$,
L.M.~Garcia~Martin$^{71}$,
J.~Garc{\'\i}a~Pardi{\~n}as$^{39}$,
J.~Garra~Tico$^{49}$,
L.~Garrido$^{38}$,
D.~Gascon$^{38}$,
C.~Gaspar$^{40}$,
L.~Gavardi$^{10}$,
G.~Gazzoni$^{5}$,
D.~Gerick$^{12}$,
E.~Gersabeck$^{56}$,
M.~Gersabeck$^{56}$,
T.~Gershon$^{50}$,
Ph.~Ghez$^{4}$,
S.~Gian{\`\i}$^{41}$,
V.~Gibson$^{49}$,
O.G.~Girard$^{41}$,
L.~Giubega$^{30}$,
K.~Gizdov$^{52}$,
V.V.~Gligorov$^{8}$,
D.~Golubkov$^{32}$,
A.~Golutvin$^{55,69,y}$,
A.~Gomes$^{1,a}$,
I.V.~Gorelov$^{33}$,
C.~Gotti$^{21,i}$,
E.~Govorkova$^{43}$,
J.P.~Grabowski$^{12}$,
R.~Graciani~Diaz$^{38}$,
L.A.~Granado~Cardoso$^{40}$,
E.~Graug{\'e}s$^{38}$,
E.~Graverini$^{42}$,
G.~Graziani$^{18}$,
A.~Grecu$^{30}$,
R.~Greim$^{9}$,
P.~Griffith$^{16}$,
L.~Grillo$^{56}$,
L.~Gruber$^{40}$,
B.R.~Gruberg~Cazon$^{57}$,
O.~Gr{\"u}nberg$^{67}$,
E.~Gushchin$^{34}$,
Yu.~Guz$^{37}$,
T.~Gys$^{40}$,
C.~G{\"o}bel$^{62}$,
T.~Hadavizadeh$^{57}$,
C.~Hadjivasiliou$^{5}$,
G.~Haefeli$^{41}$,
C.~Haen$^{40}$,
S.C.~Haines$^{49}$,
B.~Hamilton$^{60}$,
X.~Han$^{12}$,
T.H.~Hancock$^{57}$,
S.~Hansmann-Menzemer$^{12}$,
N.~Harnew$^{57}$,
S.T.~Harnew$^{48}$,
C.~Hasse$^{40}$,
M.~Hatch$^{40}$,
J.~He$^{63}$,
M.~Hecker$^{55}$,
K.~Heinicke$^{10}$,
A.~Heister$^{9}$,
K.~Hennessy$^{54}$,
P.~Henrard$^{5}$,
L.~Henry$^{71}$,
E.~van~Herwijnen$^{40}$,
M.~He{\ss}$^{67}$,
A.~Hicheur$^{2}$,
D.~Hill$^{57}$,
P.H.~Hopchev$^{41}$,
W.~Hu$^{65}$,
W.~Huang$^{63}$,
Z.C.~Huard$^{59}$,
W.~Hulsbergen$^{43}$,
T.~Humair$^{55}$,
M.~Hushchyn$^{35}$,
D.~Hutchcroft$^{54}$,
P.~Ibis$^{10}$,
M.~Idzik$^{28}$,
P.~Ilten$^{47}$,
R.~Jacobsson$^{40}$,
J.~Jalocha$^{57}$,
E.~Jans$^{43}$,
A.~Jawahery$^{60}$,
F.~Jiang$^{3}$,
M.~John$^{57}$,
D.~Johnson$^{40}$,
C.R.~Jones$^{49}$,
C.~Joram$^{40}$,
B.~Jost$^{40}$,
N.~Jurik$^{57}$,
S.~Kandybei$^{45}$,
M.~Karacson$^{40}$,
J.M.~Kariuki$^{48}$,
S.~Karodia$^{53}$,
N.~Kazeev$^{35}$,
M.~Kecke$^{12}$,
F.~Keizer$^{49}$,
M.~Kelsey$^{61}$,
M.~Kenzie$^{49}$,
T.~Ketel$^{44}$,
E.~Khairullin$^{35}$,
B.~Khanji$^{12}$,
C.~Khurewathanakul$^{41}$,
T.~Kirn$^{9}$,
S.~Klaver$^{19}$,
K.~Klimaszewski$^{29}$,
T.~Klimkovich$^{11}$,
S.~Koliiev$^{46}$,
M.~Kolpin$^{12}$,
R.~Kopecna$^{12}$,
P.~Koppenburg$^{43}$,
A.~Kosmyntseva$^{32}$,
S.~Kotriakhova$^{31}$,
M.~Kozeiha$^{5}$,
L.~Kravchuk$^{34}$,
M.~Kreps$^{50}$,
F.~Kress$^{55}$,
P.~Krokovny$^{36,w}$,
W.~Krzemien$^{29}$,
W.~Kucewicz$^{27,l}$,
M.~Kucharczyk$^{27}$,
V.~Kudryavtsev$^{36,w}$,
A.K.~Kuonen$^{41}$,
T.~Kvaratskheliya$^{32,40}$,
D.~Lacarrere$^{40}$,
G.~Lafferty$^{56}$,
A.~Lai$^{16}$,
G.~Lanfranchi$^{19}$,
C.~Langenbruch$^{9}$,
T.~Latham$^{50}$,
C.~Lazzeroni$^{47}$,
R.~Le~Gac$^{6}$,
A.~Leflat$^{33,40}$,
J.~Lefran{\c{c}}ois$^{7}$,
R.~Lef{\`e}vre$^{5}$,
F.~Lemaitre$^{40}$,
E.~Lemos~Cid$^{39}$,
O.~Leroy$^{6}$,
T.~Lesiak$^{27}$,
B.~Leverington$^{12}$,
P.-R.~Li$^{63}$,
T.~Li$^{3}$,
Y.~Li$^{7}$,
Z.~Li$^{61}$,
X.~Liang$^{61}$,
T.~Likhomanenko$^{68}$,
R.~Lindner$^{40}$,
F.~Lionetto$^{42}$,
V.~Lisovskyi$^{7}$,
X.~Liu$^{3}$,
D.~Loh$^{50}$,
A.~Loi$^{16}$,
I.~Longstaff$^{53}$,
J.H.~Lopes$^{2}$,
D.~Lucchesi$^{23,o}$,
M.~Lucio~Martinez$^{39}$,
H.~Luo$^{52}$,
A.~Lupato$^{23}$,
E.~Luppi$^{17,g}$,
O.~Lupton$^{40}$,
A.~Lusiani$^{24}$,
X.~Lyu$^{63}$,
F.~Machefert$^{7}$,
F.~Maciuc$^{30}$,
V.~Macko$^{41}$,
P.~Mackowiak$^{10}$,
S.~Maddrell-Mander$^{48}$,
O.~Maev$^{31,40}$,
K.~Maguire$^{56}$,
D.~Maisuzenko$^{31}$,
M.W.~Majewski$^{28}$,
S.~Malde$^{57}$,
B.~Malecki$^{27}$,
A.~Malinin$^{68}$,
T.~Maltsev$^{36,w}$,
G.~Manca$^{16,f}$,
G.~Mancinelli$^{6}$,
D.~Marangotto$^{22,q}$,
J.~Maratas$^{5,v}$,
J.F.~Marchand$^{4}$,
U.~Marconi$^{15}$,
C.~Marin~Benito$^{38}$,
M.~Marinangeli$^{41}$,
P.~Marino$^{41}$,
J.~Marks$^{12}$,
G.~Martellotti$^{26}$,
M.~Martin$^{6}$,
M.~Martinelli$^{41}$,
D.~Martinez~Santos$^{39}$,
F.~Martinez~Vidal$^{71}$,
A.~Massafferri$^{1}$,
R.~Matev$^{40}$,
A.~Mathad$^{50}$,
Z.~Mathe$^{40}$,
C.~Matteuzzi$^{21}$,
A.~Mauri$^{42}$,
E.~Maurice$^{7,b}$,
B.~Maurin$^{41}$,
A.~Mazurov$^{47}$,
M.~McCann$^{55,40}$,
A.~McNab$^{56}$,
R.~McNulty$^{13}$,
J.V.~Mead$^{54}$,
B.~Meadows$^{59}$,
C.~Meaux$^{6}$,
F.~Meier$^{10}$,
N.~Meinert$^{67}$,
D.~Melnychuk$^{29}$,
M.~Merk$^{43}$,
A.~Merli$^{22,40,q}$,
E.~Michielin$^{23}$,
D.A.~Milanes$^{66}$,
E.~Millard$^{50}$,
M.-N.~Minard$^{4}$,
L.~Minzoni$^{17}$,
D.S.~Mitzel$^{12}$,
A.~Mogini$^{8}$,
J.~Molina~Rodriguez$^{1}$,
T.~Momb{\"a}cher$^{10}$,
I.A.~Monroy$^{66}$,
S.~Monteil$^{5}$,
M.~Morandin$^{23}$,
M.J.~Morello$^{24,t}$,
O.~Morgunova$^{68}$,
J.~Moron$^{28}$,
A.B.~Morris$^{52}$,
R.~Mountain$^{61}$,
F.~Muheim$^{52}$,
M.~Mulder$^{43}$,
D.~M{\"u}ller$^{56}$,
J.~M{\"u}ller$^{10}$,
K.~M{\"u}ller$^{42}$,
V.~M{\"u}ller$^{10}$,
P.~Naik$^{48}$,
T.~Nakada$^{41}$,
R.~Nandakumar$^{51}$,
A.~Nandi$^{57}$,
I.~Nasteva$^{2}$,
M.~Needham$^{52}$,
N.~Neri$^{22,40}$,
S.~Neubert$^{12}$,
N.~Neufeld$^{40}$,
M.~Neuner$^{12}$,
T.D.~Nguyen$^{41}$,
C.~Nguyen-Mau$^{41,n}$,
S.~Nieswand$^{9}$,
R.~Niet$^{10}$,
N.~Nikitin$^{33}$,
T.~Nikodem$^{12}$,
A.~Nogay$^{68}$,
D.P.~O'Hanlon$^{50}$,
A.~Oblakowska-Mucha$^{28}$,
V.~Obraztsov$^{37}$,
S.~Ogilvy$^{19}$,
R.~Oldeman$^{16,f}$,
C.J.G.~Onderwater$^{72}$,
A.~Ossowska$^{27}$,
J.M.~Otalora~Goicochea$^{2}$,
P.~Owen$^{42}$,
A.~Oyanguren$^{71}$,
P.R.~Pais$^{41}$,
A.~Palano$^{14}$,
M.~Palutan$^{19,40}$,
A.~Papanestis$^{51}$,
M.~Pappagallo$^{52}$,
L.L.~Pappalardo$^{17,g}$,
W.~Parker$^{60}$,
C.~Parkes$^{56}$,
G.~Passaleva$^{18,40}$,
A.~Pastore$^{14,d}$,
M.~Patel$^{55}$,
C.~Patrignani$^{15,e}$,
A.~Pellegrino$^{43}$,
G.~Penso$^{26}$,
M.~Pepe~Altarelli$^{40}$,
S.~Perazzini$^{40}$,
D.~Pereima$^{32}$,
P.~Perret$^{5}$,
L.~Pescatore$^{41}$,
K.~Petridis$^{48}$,
A.~Petrolini$^{20,h}$,
A.~Petrov$^{68}$,
M.~Petruzzo$^{22,q}$,
E.~Picatoste~Olloqui$^{38}$,
B.~Pietrzyk$^{4}$,
G.~Pietrzyk$^{41}$,
M.~Pikies$^{27}$,
D.~Pinci$^{26}$,
F.~Pisani$^{40}$,
A.~Pistone$^{20,h}$,
A.~Piucci$^{12}$,
V.~Placinta$^{30}$,
S.~Playfer$^{52}$,
M.~Plo~Casasus$^{39}$,
F.~Polci$^{8}$,
M.~Poli~Lener$^{19}$,
A.~Poluektov$^{50}$,
I.~Polyakov$^{61}$,
E.~Polycarpo$^{2}$,
G.J.~Pomery$^{48}$,
S.~Ponce$^{40}$,
A.~Popov$^{37}$,
D.~Popov$^{11,40}$,
S.~Poslavskii$^{37}$,
C.~Potterat$^{2}$,
E.~Price$^{48}$,
J.~Prisciandaro$^{39}$,
C.~Prouve$^{48}$,
V.~Pugatch$^{46}$,
A.~Puig~Navarro$^{42}$,
H.~Pullen$^{57}$,
G.~Punzi$^{24,p}$,
W.~Qian$^{50}$,
J.~Qin$^{63}$,
R.~Quagliani$^{8}$,
B.~Quintana$^{5}$,
B.~Rachwal$^{28}$,
J.H.~Rademacker$^{48}$,
M.~Rama$^{24}$,
M.~Ramos~Pernas$^{39}$,
M.S.~Rangel$^{2}$,
I.~Raniuk$^{45,\dagger}$,
F.~Ratnikov$^{35,x}$,
G.~Raven$^{44}$,
M.~Ravonel~Salzgeber$^{40}$,
M.~Reboud$^{4}$,
F.~Redi$^{41}$,
S.~Reichert$^{10}$,
A.C.~dos~Reis$^{1}$,
C.~Remon~Alepuz$^{71}$,
V.~Renaudin$^{7}$,
S.~Ricciardi$^{51}$,
S.~Richards$^{48}$,
M.~Rihl$^{40}$,
K.~Rinnert$^{54}$,
P.~Robbe$^{7}$,
A.~Robert$^{8}$,
A.B.~Rodrigues$^{41}$,
E.~Rodrigues$^{59}$,
J.A.~Rodriguez~Lopez$^{66}$,
A.~Rogozhnikov$^{35}$,
S.~Roiser$^{40}$,
A.~Rollings$^{57}$,
V.~Romanovskiy$^{37}$,
A.~Romero~Vidal$^{39,40}$,
M.~Rotondo$^{19}$,
M.S.~Rudolph$^{61}$,
T.~Ruf$^{40}$,
P.~Ruiz~Valls$^{71}$,
J.~Ruiz~Vidal$^{71}$,
J.J.~Saborido~Silva$^{39}$,
E.~Sadykhov$^{32}$,
N.~Sagidova$^{31}$,
B.~Saitta$^{16,f}$,
V.~Salustino~Guimaraes$^{62}$,
C.~Sanchez~Mayordomo$^{71}$,
B.~Sanmartin~Sedes$^{39}$,
R.~Santacesaria$^{26}$,
C.~Santamarina~Rios$^{39}$,
M.~Santimaria$^{19}$,
E.~Santovetti$^{25,j}$,
G.~Sarpis$^{56}$,
A.~Sarti$^{19,k}$,
C.~Satriano$^{26,s}$,
A.~Satta$^{25}$,
D.M.~Saunders$^{48}$,
D.~Savrina$^{32,33}$,
S.~Schael$^{9}$,
M.~Schellenberg$^{10}$,
M.~Schiller$^{53}$,
H.~Schindler$^{40}$,
M.~Schmelling$^{11}$,
T.~Schmelzer$^{10}$,
B.~Schmidt$^{40}$,
O.~Schneider$^{41}$,
A.~Schopper$^{40}$,
H.F.~Schreiner$^{59}$,
M.~Schubiger$^{41}$,
M.H.~Schune$^{7}$,
R.~Schwemmer$^{40}$,
B.~Sciascia$^{19}$,
A.~Sciubba$^{26,k}$,
A.~Semennikov$^{32}$,
E.S.~Sepulveda$^{8}$,
A.~Sergi$^{47}$,
N.~Serra$^{42}$,
J.~Serrano$^{6}$,
L.~Sestini$^{23}$,
P.~Seyfert$^{40}$,
M.~Shapkin$^{37}$,
I.~Shapoval$^{45}$,
Y.~Shcheglov$^{31}$,
T.~Shears$^{54}$,
L.~Shekhtman$^{36,w}$,
V.~Shevchenko$^{68}$,
B.G.~Siddi$^{17}$,
R.~Silva~Coutinho$^{42}$,
L.~Silva~de~Oliveira$^{2}$,
G.~Simi$^{23,o}$,
S.~Simone$^{14,d}$,
M.~Sirendi$^{49}$,
N.~Skidmore$^{48}$,
T.~Skwarnicki$^{61}$,
I.T.~Smith$^{52}$,
J.~Smith$^{49}$,
M.~Smith$^{55}$,
l.~Soares~Lavra$^{1}$,
M.D.~Sokoloff$^{59}$,
F.J.P.~Soler$^{53}$,
B.~Souza~De~Paula$^{2}$,
B.~Spaan$^{10}$,
P.~Spradlin$^{53}$,
S.~Sridharan$^{40}$,
F.~Stagni$^{40}$,
M.~Stahl$^{12}$,
S.~Stahl$^{40}$,
P.~Stefko$^{41}$,
S.~Stefkova$^{55}$,
O.~Steinkamp$^{42}$,
S.~Stemmle$^{12}$,
O.~Stenyakin$^{37}$,
M.~Stepanova$^{31}$,
H.~Stevens$^{10}$,
S.~Stone$^{61}$,
B.~Storaci$^{42}$,
S.~Stracka$^{24,p}$,
M.E.~Stramaglia$^{41}$,
M.~Straticiuc$^{30}$,
U.~Straumann$^{42}$,
J.~Sun$^{3}$,
L.~Sun$^{64}$,
K.~Swientek$^{28}$,
V.~Syropoulos$^{44}$,
T.~Szumlak$^{28}$,
M.~Szymanski$^{63}$,
S.~T'Jampens$^{4}$,
A.~Tayduganov$^{6}$,
T.~Tekampe$^{10}$,
G.~Tellarini$^{17,g}$,
F.~Teubert$^{40}$,
E.~Thomas$^{40}$,
J.~van~Tilburg$^{43}$,
M.J.~Tilley$^{55}$,
V.~Tisserand$^{5}$,
M.~Tobin$^{41}$,
S.~Tolk$^{49}$,
L.~Tomassetti$^{17,g}$,
D.~Tonelli$^{24}$,
R.~Tourinho~Jadallah~Aoude$^{1}$,
E.~Tournefier$^{4}$,
M.~Traill$^{53}$,
M.T.~Tran$^{41}$,
M.~Tresch$^{42}$,
A.~Trisovic$^{49}$,
A.~Tsaregorodtsev$^{6}$,
P.~Tsopelas$^{43}$,
A.~Tully$^{49}$,
N.~Tuning$^{43,40}$,
A.~Ukleja$^{29}$,
A.~Usachov$^{7}$,
A.~Ustyuzhanin$^{35}$,
U.~Uwer$^{12}$,
C.~Vacca$^{16,f}$,
A.~Vagner$^{70}$,
V.~Vagnoni$^{15,40}$,
A.~Valassi$^{40}$,
S.~Valat$^{40}$,
G.~Valenti$^{15}$,
R.~Vazquez~Gomez$^{40}$,
P.~Vazquez~Regueiro$^{39}$,
S.~Vecchi$^{17}$,
M.~van~Veghel$^{43}$,
J.J.~Velthuis$^{48}$,
M.~Veltri$^{18,r}$,
G.~Veneziano$^{57}$,
A.~Venkateswaran$^{61}$,
T.A.~Verlage$^{9}$,
M.~Vernet$^{5}$,
M.~Vesterinen$^{57}$,
J.V.~Viana~Barbosa$^{40}$,
D.~~Vieira$^{63}$,
M.~Vieites~Diaz$^{39}$,
H.~Viemann$^{67}$,
X.~Vilasis-Cardona$^{38,m}$,
M.~Vitti$^{49}$,
V.~Volkov$^{33}$,
A.~Vollhardt$^{42}$,
B.~Voneki$^{40}$,
A.~Vorobyev$^{31}$,
V.~Vorobyev$^{36,w}$,
C.~Vo{\ss}$^{9}$,
J.A.~de~Vries$^{43}$,
C.~V{\'a}zquez~Sierra$^{43}$,
R.~Waldi$^{67}$,
J.~Walsh$^{24}$,
J.~Wang$^{61}$,
Y.~Wang$^{65}$,
D.R.~Ward$^{49}$,
H.M.~Wark$^{54}$,
N.K.~Watson$^{47}$,
D.~Websdale$^{55}$,
A.~Weiden$^{42}$,
C.~Weisser$^{58}$,
M.~Whitehead$^{40}$,
J.~Wicht$^{50}$,
G.~Wilkinson$^{57}$,
M.~Wilkinson$^{61}$,
M.~Williams$^{56}$,
M.~Williams$^{58}$,
T.~Williams$^{47}$,
F.F.~Wilson$^{51,40}$,
J.~Wimberley$^{60}$,
M.~Winn$^{7}$,
J.~Wishahi$^{10}$,
W.~Wislicki$^{29}$,
M.~Witek$^{27}$,
G.~Wormser$^{7}$,
S.A.~Wotton$^{49}$,
K.~Wyllie$^{40}$,
Y.~Xie$^{65}$,
M.~Xu$^{65}$,
Q.~Xu$^{63}$,
Z.~Xu$^{3}$,
Z.~Xu$^{4}$,
Z.~Yang$^{3}$,
Z.~Yang$^{60}$,
Y.~Yao$^{61}$,
H.~Yin$^{65}$,
J.~Yu$^{65}$,
X.~Yuan$^{61}$,
O.~Yushchenko$^{37}$,
K.A.~Zarebski$^{47}$,
M.~Zavertyaev$^{11,c}$,
L.~Zhang$^{3}$,
Y.~Zhang$^{7}$,
A.~Zhelezov$^{12}$,
Y.~Zheng$^{63}$,
X.~Zhu$^{3}$,
V.~Zhukov$^{9,33}$,
J.B.~Zonneveld$^{52}$,
S.~Zucchelli$^{15}$.\bigskip

{\footnotesize \it
$ ^{1}$Centro Brasileiro de Pesquisas F{\'\i}sicas (CBPF), Rio de Janeiro, Brazil\\
$ ^{2}$Universidade Federal do Rio de Janeiro (UFRJ), Rio de Janeiro, Brazil\\
$ ^{3}$Center for High Energy Physics, Tsinghua University, Beijing, China\\
$ ^{4}$Univ. Grenoble Alpes, Univ. Savoie Mont Blanc, CNRS, IN2P3-LAPP, Annecy, France\\
$ ^{5}$Clermont Universit{\'e}, Universit{\'e} Blaise Pascal, CNRS/IN2P3, LPC, Clermont-Ferrand, France\\
$ ^{6}$Aix Marseille Univ, CNRS/IN2P3, CPPM, Marseille, France\\
$ ^{7}$LAL, Univ. Paris-Sud, CNRS/IN2P3, Universit{\'e} Paris-Saclay, Orsay, France\\
$ ^{8}$LPNHE, Universit{\'e} Pierre et Marie Curie, Universit{\'e} Paris Diderot, CNRS/IN2P3, Paris, France\\
$ ^{9}$I. Physikalisches Institut, RWTH Aachen University, Aachen, Germany\\
$ ^{10}$Fakult{\"a}t Physik, Technische Universit{\"a}t Dortmund, Dortmund, Germany\\
$ ^{11}$Max-Planck-Institut f{\"u}r Kernphysik (MPIK), Heidelberg, Germany\\
$ ^{12}$Physikalisches Institut, Ruprecht-Karls-Universit{\"a}t Heidelberg, Heidelberg, Germany\\
$ ^{13}$School of Physics, University College Dublin, Dublin, Ireland\\
$ ^{14}$Sezione INFN di Bari, Bari, Italy\\
$ ^{15}$Sezione INFN di Bologna, Bologna, Italy\\
$ ^{16}$Sezione INFN di Cagliari, Cagliari, Italy\\
$ ^{17}$Universita e INFN, Ferrara, Ferrara, Italy\\
$ ^{18}$Sezione INFN di Firenze, Firenze, Italy\\
$ ^{19}$Laboratori Nazionali dell'INFN di Frascati, Frascati, Italy\\
$ ^{20}$Sezione INFN di Genova, Genova, Italy\\
$ ^{21}$Sezione INFN di Milano Bicocca, Milano, Italy\\
$ ^{22}$Sezione di Milano, Milano, Italy\\
$ ^{23}$Sezione INFN di Padova, Padova, Italy\\
$ ^{24}$Sezione INFN di Pisa, Pisa, Italy\\
$ ^{25}$Sezione INFN di Roma Tor Vergata, Roma, Italy\\
$ ^{26}$Sezione INFN di Roma La Sapienza, Roma, Italy\\
$ ^{27}$Henryk Niewodniczanski Institute of Nuclear Physics  Polish Academy of Sciences, Krak{\'o}w, Poland\\
$ ^{28}$AGH - University of Science and Technology, Faculty of Physics and Applied Computer Science, Krak{\'o}w, Poland\\
$ ^{29}$National Center for Nuclear Research (NCBJ), Warsaw, Poland\\
$ ^{30}$Horia Hulubei National Institute of Physics and Nuclear Engineering, Bucharest-Magurele, Romania\\
$ ^{31}$Petersburg Nuclear Physics Institute (PNPI), Gatchina, Russia\\
$ ^{32}$Institute of Theoretical and Experimental Physics (ITEP), Moscow, Russia\\
$ ^{33}$Institute of Nuclear Physics, Moscow State University (SINP MSU), Moscow, Russia\\
$ ^{34}$Institute for Nuclear Research of the Russian Academy of Sciences (INR RAS), Moscow, Russia\\
$ ^{35}$Yandex School of Data Analysis, Moscow, Russia\\
$ ^{36}$Budker Institute of Nuclear Physics (SB RAS), Novosibirsk, Russia\\
$ ^{37}$Institute for High Energy Physics (IHEP), Protvino, Russia\\
$ ^{38}$ICCUB, Universitat de Barcelona, Barcelona, Spain\\
$ ^{39}$Instituto Galego de F{\'\i}sica de Altas Enerx{\'\i}as (IGFAE), Universidade de Santiago de Compostela, Santiago de Compostela, Spain\\
$ ^{40}$European Organization for Nuclear Research (CERN), Geneva, Switzerland\\
$ ^{41}$Institute of Physics, Ecole Polytechnique  F{\'e}d{\'e}rale de Lausanne (EPFL), Lausanne, Switzerland\\
$ ^{42}$Physik-Institut, Universit{\"a}t Z{\"u}rich, Z{\"u}rich, Switzerland\\
$ ^{43}$Nikhef National Institute for Subatomic Physics, Amsterdam, The Netherlands\\
$ ^{44}$Nikhef National Institute for Subatomic Physics and VU University Amsterdam, Amsterdam, The Netherlands\\
$ ^{45}$NSC Kharkiv Institute of Physics and Technology (NSC KIPT), Kharkiv, Ukraine\\
$ ^{46}$Institute for Nuclear Research of the National Academy of Sciences (KINR), Kyiv, Ukraine\\
$ ^{47}$University of Birmingham, Birmingham, United Kingdom\\
$ ^{48}$H.H. Wills Physics Laboratory, University of Bristol, Bristol, United Kingdom\\
$ ^{49}$Cavendish Laboratory, University of Cambridge, Cambridge, United Kingdom\\
$ ^{50}$Department of Physics, University of Warwick, Coventry, United Kingdom\\
$ ^{51}$STFC Rutherford Appleton Laboratory, Didcot, United Kingdom\\
$ ^{52}$School of Physics and Astronomy, University of Edinburgh, Edinburgh, United Kingdom\\
$ ^{53}$School of Physics and Astronomy, University of Glasgow, Glasgow, United Kingdom\\
$ ^{54}$Oliver Lodge Laboratory, University of Liverpool, Liverpool, United Kingdom\\
$ ^{55}$Imperial College London, London, United Kingdom\\
$ ^{56}$School of Physics and Astronomy, University of Manchester, Manchester, United Kingdom\\
$ ^{57}$Department of Physics, University of Oxford, Oxford, United Kingdom\\
$ ^{58}$Massachusetts Institute of Technology, Cambridge, MA, United States\\
$ ^{59}$University of Cincinnati, Cincinnati, OH, United States\\
$ ^{60}$University of Maryland, College Park, MD, United States\\
$ ^{61}$Syracuse University, Syracuse, NY, United States\\
$ ^{62}$Pontif{\'\i}cia Universidade Cat{\'o}lica do Rio de Janeiro (PUC-Rio), Rio de Janeiro, Brazil, associated to $^{2}$\\
$ ^{63}$University of Chinese Academy of Sciences, Beijing, China, associated to $^{3}$\\
$ ^{64}$School of Physics and Technology, Wuhan University, Wuhan, China, associated to $^{3}$\\
$ ^{65}$Institute of Particle Physics, Central China Normal University, Wuhan, Hubei, China, associated to $^{3}$\\
$ ^{66}$Departamento de Fisica , Universidad Nacional de Colombia, Bogota, Colombia, associated to $^{8}$\\
$ ^{67}$Institut f{\"u}r Physik, Universit{\"a}t Rostock, Rostock, Germany, associated to $^{12}$\\
$ ^{68}$National Research Centre Kurchatov Institute, Moscow, Russia, associated to $^{32}$\\
$ ^{69}$National University of Science and Technology MISIS, Moscow, Russia, associated to $^{32}$\\
$ ^{70}$National Research Tomsk Polytechnic University, Tomsk, Russia, associated to $^{32}$\\
$ ^{71}$Instituto de Fisica Corpuscular, Centro Mixto Universidad de Valencia - CSIC, Valencia, Spain, associated to $^{38}$\\
$ ^{72}$Van Swinderen Institute, University of Groningen, Groningen, The Netherlands, associated to $^{43}$\\
$ ^{73}$Los Alamos National Laboratory (LANL), Los Alamos, United States, associated to $^{61}$\\
\bigskip
$ ^{a}$Universidade Federal do Tri{\^a}ngulo Mineiro (UFTM), Uberaba-MG, Brazil\\
$ ^{b}$Laboratoire Leprince-Ringuet, Palaiseau, France\\
$ ^{c}$P.N. Lebedev Physical Institute, Russian Academy of Science (LPI RAS), Moscow, Russia\\
$ ^{d}$Universit{\`a} di Bari, Bari, Italy\\
$ ^{e}$Universit{\`a} di Bologna, Bologna, Italy\\
$ ^{f}$Universit{\`a} di Cagliari, Cagliari, Italy\\
$ ^{g}$Universit{\`a} di Ferrara, Ferrara, Italy\\
$ ^{h}$Universit{\`a} di Genova, Genova, Italy\\
$ ^{i}$Universit{\`a} di Milano Bicocca, Milano, Italy\\
$ ^{j}$Universit{\`a} di Roma Tor Vergata, Roma, Italy\\
$ ^{k}$Universit{\`a} di Roma La Sapienza, Roma, Italy\\
$ ^{l}$AGH - University of Science and Technology, Faculty of Computer Science, Electronics and Telecommunications, Krak{\'o}w, Poland\\
$ ^{m}$LIFAELS, La Salle, Universitat Ramon Llull, Barcelona, Spain\\
$ ^{n}$Hanoi University of Science, Hanoi, Vietnam\\
$ ^{o}$Universit{\`a} di Padova, Padova, Italy\\
$ ^{p}$Universit{\`a} di Pisa, Pisa, Italy\\
$ ^{q}$Universit{\`a} degli Studi di Milano, Milano, Italy\\
$ ^{r}$Universit{\`a} di Urbino, Urbino, Italy\\
$ ^{s}$Universit{\`a} della Basilicata, Potenza, Italy\\
$ ^{t}$Scuola Normale Superiore, Pisa, Italy\\
$ ^{u}$Universit{\`a} di Modena e Reggio Emilia, Modena, Italy\\
$ ^{v}$Iligan Institute of Technology (IIT), Iligan, Philippines\\
$ ^{w}$Novosibirsk State University, Novosibirsk, Russia\\
$ ^{x}$National Research University Higher School of Economics, Moscow, Russia\\
$ ^{y}$National University of Science and Technology MISIS, Moscow, Russia\\
\medskip
$ ^{\dagger}$Deceased
}
\end{flushleft}

==> lhcb-symbols-def.tex <==
%%% $Id: lhcb-symbols-def.tex 82618 2015-10-14 14:53:43Z pkoppenb $
%%% ======================================================================
%%% Purpose: Standard LHCb aliases
%%% Author: Originally Ulrik Egede, adapted by Tomasz Skwarnicki for templates,
%%% rewritten by Chris Parkes
%%% Maintainer : Ulrik Egede (2010 - 2012)
%%% Maintainer : Rolf Oldeman (2012 - 2014)
%%% =======================================================================

%%% To use this file outside the normal LHCb document environment, the
%%% following should be added in a preamble (before \begin{document}
%%%
%%%\usepackage{ifthen} 
%%%\newboolean{uprightparticles}
%%%\setboolean{uprightparticles}{false} %Set true for upright particle symbols
\usepackage{xspace} 
\usepackage{upgreek}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%
%%% The following is to ensure that the template automatically can process
%%% this file.
%%%
%%% Add comments with at least three %%% preceding.
%%% Add new sections with one % preceding
%%% Add new subsections with two %% preceding
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%
% Experiments
%%%%%%%%%%%%%
\def\lhcb {\mbox{LHCb}\xspace}
\def\atlas  {\mbox{ATLAS}\xspace}
\def\cms    {\mbox{CMS}\xspace}
\def\alice  {\mbox{ALICE}\xspace}
\def\babar  {\mbox{BaBar}\xspace}
\def\belle  {\mbox{Belle}\xspace}
\def\cleo   {\mbox{CLEO}\xspace}
\def\cdf    {\mbox{CDF}\xspace}
\def\dzero  {\mbox{D0}\xspace}
\def\aleph  {\mbox{ALEPH}\xspace}
\def\delphi {\mbox{DELPHI}\xspace}
\def\opal   {\mbox{OPAL}\xspace}
\def\lthree {\mbox{L3}\xspace}
\def\sld    {\mbox{SLD}\xspace}
%%%\def\argus  {\mbox{ARGUS}\xspace}
%%%\def\uaone  {\mbox{UA1}\xspace}
%%%\def\uatwo  {\mbox{UA2}\xspace}
%%%\def\ux85 {\mbox{UX85}\xspace}
\def\cern {\mbox{CERN}\xspace}
\def\lhc    {\mbox{LHC}\xspace}
\def\lep    {\mbox{LEP}\xspace}
\def\tevatron {Tevatron\xspace}

%% LHCb sub-detectors and sub-systems

%%%\def\pu     {PU\xspace}
\def\velo   {VELO\xspace}
\def\rich   {RICH\xspace}
\def\richone {RICH1\xspace}
\def\richtwo {RICH2\xspace}
\def\ttracker {TT\xspace}
\def\intr   {IT\xspace}
\def\st     {ST\xspace}
\def\ot     {OT\xspace}
%%%\def\Tone   {T1\xspace}
%%%\def\Ttwo   {T2\xspace}
%%%\def\Tthree {T3\xspace}
%%%\def\Mone   {M1\xspace}
%%%\def\Mtwo   {M2\xspace}
%%%\def\Mthree {M3\xspace}
%%%\def\Mfour  {M4\xspace}
%%%\def\Mfive  {M5\xspace}
\def\spd    {SPD\xspace}
\def\presh  {PS\xspace}
\def\ecal   {ECAL\xspace}
\def\hcal   {HCAL\xspace}
%%%\def\bcm    {BCM\xspace}
\def\MagUp {\mbox{\em Mag\kern -0.05em Up}\xspace}
\def\MagDown {\mbox{\em MagDown}\xspace}

\def\ode    {ODE\xspace}
\def\daq    {DAQ\xspace}
\def\tfc    {TFC\xspace}
\def\ecs    {ECS\xspace}
\def\lone   {L0\xspace}
\def\hlt    {HLT\xspace}
\def\hltone {HLT1\xspace}
\def\hlttwo {HLT2\xspace}

%%% Upright (not slanted) Particles

\ifthenelse{\boolean{uprightparticles}}%
{\def\Palpha      {\ensuremath{\upalpha}\xspace}
 \def\Pbeta       {\ensuremath{\upbeta}\xspace}
 \def\Pgamma      {\ensuremath{\upgamma}\xspace}                 
 \def\Pdelta      {\ensuremath{\updelta}\xspace}                 
 \def\Pepsilon    {\ensuremath{\upepsilon}\xspace}                 
 \def\Pvarepsilon {\ensuremath{\upvarepsilon}\xspace}                 
 \def\Pzeta       {\ensuremath{\upzeta}\xspace}                 
 \def\Peta        {\ensuremath{\upeta}\xspace}                 
 \def\Ptheta      {\ensuremath{\uptheta}\xspace}                 
 \def\Pvartheta   {\ensuremath{\upvartheta}\xspace}                 
 \def\Piota       {\ensuremath{\upiota}\xspace}                 
 \def\Pkappa      {\ensuremath{\upkappa}\xspace}                 
 \def\Plambda     {\ensuremath{\uplambda}\xspace}                 
 \def\Pmu         {\ensuremath{\upmu}\xspace}                 
 \def\Pnu         {\ensuremath{\upnu}\xspace}                 
 \def\Pxi         {\ensuremath{\upxi}\xspace}                 
 \def\Ppi         {\ensuremath{\uppi}\xspace}                 
 \def\Pvarpi      {\ensuremath{\upvarpi}\xspace}                 
 \def\Prho        {\ensuremath{\uprho}\xspace}                 
 \def\Pvarrho     {\ensuremath{\upvarrho}\xspace}                 
 \def\Ptau        {\ensuremath{\uptau}\xspace}                 
 \def\Pupsilon    {\ensuremath{\upupsilon}\xspace}                 
 \def\Pphi        {\ensuremath{\upphi}\xspace}                 
 \def\Pvarphi     {\ensuremath{\upvarphi}\xspace}                 
 \def\Pchi        {\ensuremath{\upchi}\xspace}                 
 \def\Ppsi        {\ensuremath{\uppsi}\xspace}                 
 \def\Pomega      {\ensuremath{\upomega}\xspace}                 


 \def\PDelta      {\ensuremath{\Delta}\xspace}                 
 \def\PXi      {\ensuremath{\Xi}\xspace}                 
 \def\PLambda      {\ensuremath{\Lambda}\xspace}                 
 \def\PSigma      {\ensuremath{\Sigma}\xspace}                 
 \def\POmega      {\ensuremath{\Omega}\xspace}                 
 \def\PUpsilon      {\ensuremath{\Upsilon}\xspace}                 
 
 %\mathchardef\Deltares="7101
 %\mathchardef\Xi="7104
 %\mathchardef\Lambda="7103
 %\mathchardef\Sigma="7106
 %\mathchardef\Omega="710A


 \def\PA      {\ensuremath{\mathrm{A}}\xspace}                 
 \def\PB      {\ensuremath{\mathrm{B}}\xspace}                 
 \def\PC      {\ensuremath{\mathrm{C}}\xspace}                 
 \def\PD      {\ensuremath{\mathrm{D}}\xspace}                 
 \def\PE      {\ensuremath{\mathrm{E}}\xspace}                 
 \def\PF      {\ensuremath{\mathrm{F}}\xspace}                 
 \def\PG      {\ensuremath{\mathrm{G}}\xspace}                 
 \def\PH      {\ensuremath{\mathrm{H}}\xspace}                 
 \def\PI      {\ensuremath{\mathrm{I}}\xspace}                 
 \def\PJ      {\ensuremath{\mathrm{J}}\xspace}                 
 \def\PK      {\ensuremath{\mathrm{K}}\xspace}                 
 \def\PL      {\ensuremath{\mathrm{L}}\xspace}                 
 \def\PM      {\ensuremath{\mathrm{M}}\xspace}                 
 \def\PN      {\ensuremath{\mathrm{N}}\xspace}                 
 \def\PO      {\ensuremath{\mathrm{O}}\xspace}                 
 \def\PP      {\ensuremath{\mathrm{P}}\xspace}                 
 \def\PQ      {\ensuremath{\mathrm{Q}}\xspace}                 
 \def\PR      {\ensuremath{\mathrm{R}}\xspace}                 
 \def\PS      {\ensuremath{\mathrm{S}}\xspace}                 
 \def\PT      {\ensuremath{\mathrm{T}}\xspace}                 
 \def\PU      {\ensuremath{\mathrm{U}}\xspace}                 
 \def\PV      {\ensuremath{\mathrm{V}}\xspace}                 
 \def\PW      {\ensuremath{\mathrm{W}}\xspace}                 
 \def\PX      {\ensuremath{\mathrm{X}}\xspace}                 
 \def\PY      {\ensuremath{\mathrm{Y}}\xspace}                 
 \def\PZ      {\ensuremath{\mathrm{Z}}\xspace}                 
 \def\Pa      {\ensuremath{\mathrm{a}}\xspace}                 
 \def\Pb      {\ensuremath{\mathrm{b}}\xspace}                 
 \def\Pc      {\ensuremath{\mathrm{c}}\xspace}                 
 \def\Pd      {\ensuremath{\mathrm{d}}\xspace}                 
 \def\Pe      {\ensuremath{\mathrm{e}}\xspace}                 
 \def\Pf      {\ensuremath{\mathrm{f}}\xspace}                 
 \def\Pg      {\ensuremath{\mathrm{g}}\xspace}                 
 \def\Ph      {\ensuremath{\mathrm{h}}\xspace}                 
 \def\Pi      {\ensuremath{\mathrm{i}}\xspace}                 
 \def\Pj      {\ensuremath{\mathrm{j}}\xspace}                 
 \def\Pk      {\ensuremath{\mathrm{k}}\xspace}                 
 \def\Pl      {\ensuremath{\mathrm{l}}\xspace}                 
 \def\Pm      {\ensuremath{\mathrm{m}}\xspace}                 
 \def\Pn      {\ensuremath{\mathrm{n}}\xspace}                 
 \def\Po      {\ensuremath{\mathrm{o}}\xspace}                 
 \def\Pp      {\ensuremath{\mathrm{p}}\xspace}                 
 \def\Pq      {\ensuremath{\mathrm{q}}\xspace}                 
 \def\Pr      {\ensuremath{\mathrm{r}}\xspace}                 
 \def\Ps      {\ensuremath{\mathrm{s}}\xspace}                 
 \def\Pt      {\ensuremath{\mathrm{t}}\xspace}                 
 \def\Pu      {\ensuremath{\mathrm{u}}\xspace}                 
 \def\Pv      {\ensuremath{\mathrm{v}}\xspace}                 
 \def\Pw      {\ensuremath{\mathrm{w}}\xspace}                 
 \def\Px      {\ensuremath{\mathrm{x}}\xspace}                 
 \def\Py      {\ensuremath{\mathrm{y}}\xspace}                 
 \def\Pz      {\ensuremath{\mathrm{z}}\xspace}                 
}
{\def\Palpha      {\ensuremath{\alpha}\xspace}
 \def\Pbeta       {\ensuremath{\beta}\xspace}
 \def\Pgamma      {\ensuremath{\gamma}\xspace}                 
 \def\Pdelta      {\ensuremath{\delta}\xspace}                 
 \def\Pepsilon    {\ensuremath{\epsilon}\xspace}                 
 \def\Pvarepsilon {\ensuremath{\varepsilon}\xspace}                 
 \def\Pzeta       {\ensuremath{\zeta}\xspace}                 
 \def\Peta        {\ensuremath{\eta}\xspace}                 
 \def\Ptheta      {\ensuremath{\theta}\xspace}                 
 \def\Pvartheta   {\ensuremath{\vartheta}\xspace}                 
 \def\Piota       {\ensuremath{\iota}\xspace}                 
 \def\Pkappa      {\ensuremath{\kappa}\xspace}                 
 \def\Plambda     {\ensuremath{\lambda}\xspace}                 
 \def\Pmu         {\ensuremath{\mu}\xspace}                 
 \def\Pnu         {\ensuremath{\nu}\xspace}                 
 \def\Pxi         {\ensuremath{\xi}\xspace}                 
 \def\Ppi         {\ensuremath{\pi}\xspace}                 
 \def\Pvarpi      {\ensuremath{\varpi}\xspace}                 
 \def\Prho        {\ensuremath{\rho}\xspace}                 
 \def\Pvarrho     {\ensuremath{\varrho}\xspace}                 
 \def\Ptau        {\ensuremath{\tau}\xspace}                 
 \def\Pupsilon    {\ensuremath{\upsilon}\xspace}                 
 \def\Pphi        {\ensuremath{\phi}\xspace}                 
 \def\Pvarphi     {\ensuremath{\varphi}\xspace}                 
 \def\Pchi        {\ensuremath{\chi}\xspace}                 
 \def\Ppsi        {\ensuremath{\psi}\xspace}                 
 \def\Pomega      {\ensuremath{\omega}\xspace}                 
 \mathchardef\PDelta="7101
 \mathchardef\PXi="7104
 \mathchardef\PLambda="7103
 \mathchardef\PSigma="7106
 \mathchardef\POmega="710A
 \mathchardef\PUpsilon="7107
 \def\PA      {\ensuremath{A}\xspace}                 
 \def\PB      {\ensuremath{B}\xspace}                 
 \def\PC      {\ensuremath{C}\xspace}                 
 \def\PD      {\ensuremath{D}\xspace}                 
 \def\PE      {\ensuremath{E}\xspace}                 
 \def\PF      {\ensuremath{F}\xspace}                 
 \def\PG      {\ensuremath{G}\xspace}                 
 \def\PH      {\ensuremath{H}\xspace}                 
 \def\PI      {\ensuremath{I}\xspace}                 
 \def\PJ      {\ensuremath{J}\xspace}                 
 \def\PK      {\ensuremath{K}\xspace}                 
 \def\PL      {\ensuremath{L}\xspace}                 
 \def\PM      {\ensuremath{M}\xspace}                 
 \def\PN      {\ensuremath{N}\xspace}                 
 \def\PO      {\ensuremath{O}\xspace}                 
 \def\PP      {\ensuremath{P}\xspace}                 
 \def\PQ      {\ensuremath{Q}\xspace}                 
 \def\PR      {\ensuremath{R}\xspace}                 
 \def\PS      {\ensuremath{S}\xspace}                 
 \def\PT      {\ensuremath{T}\xspace}                 
 \def\PU      {\ensuremath{U}\xspace}                 
 \def\PV      {\ensuremath{V}\xspace}                 
 \def\PW      {\ensuremath{W}\xspace}                 
 \def\PX      {\ensuremath{X}\xspace}                 
 \def\PY      {\ensuremath{Y}\xspace}                 
 \def\PZ      {\ensuremath{Z}\xspace}                 
 \def\Pa      {\ensuremath{a}\xspace}                 
 \def\Pb      {\ensuremath{b}\xspace}                 
 \def\Pc      {\ensuremath{c}\xspace}                 
 \def\Pd      {\ensuremath{d}\xspace}                 
 \def\Pe      {\ensuremath{e}\xspace}                 
 \def\Pf      {\ensuremath{f}\xspace}                 
 \def\Pg      {\ensuremath{g}\xspace}                 
 \def\Ph      {\ensuremath{h}\xspace}                 
 \def\Pi      {\ensuremath{i}\xspace}                 
 \def\Pj      {\ensuremath{j}\xspace}                 
 \def\Pk      {\ensuremath{k}\xspace}                 
 \def\Pl      {\ensuremath{l}\xspace}                 
 \def\Pm      {\ensuremath{m}\xspace}                 
 \def\Pn      {\ensuremath{n}\xspace}                 
 \def\Po      {\ensuremath{o}\xspace}                 
 \def\Pp      {\ensuremath{p}\xspace}                 
 \def\Pq      {\ensuremath{q}\xspace}                 
 \def\Pr      {\ensuremath{r}\xspace}                 
 \def\Ps      {\ensuremath{s}\xspace}                 
 \def\Pt      {\ensuremath{t}\xspace}                 
 \def\Pu      {\ensuremath{u}\xspace}                 
 \def\Pv      {\ensuremath{v}\xspace}                 
 \def\Pw      {\ensuremath{w}\xspace}                 
 \def\Px      {\ensuremath{x}\xspace}                 
 \def\Py      {\ensuremath{y}\xspace}                 
 \def\Pz      {\ensuremath{z}\xspace}                 
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Particles
\makeatletter
\ifcase \@ptsize \relax% 10pt
  \newcommand{\miniscule}{\@setfontsize\miniscule{4}{5}}% \tiny: 5/6
\or% 11pt
  \newcommand{\miniscule}{\@setfontsize\miniscule{5}{6}}% \tiny: 6/7
\or% 12pt
  \newcommand{\miniscule}{\@setfontsize\miniscule{5}{6}}% \tiny: 6/7
\fi
\makeatother


\DeclareRobustCommand{\optbar}[1]{\shortstack{{\miniscule (\rule[.5ex]{1.25em}{.18mm})}
  \\ [-.7ex] $#1$}}


%% Leptons

\let\emi\en
\def\electron   {{\ensuremath{\Pe}}\xspace}
\def\en         {{\ensuremath{\Pe^-}}\xspace}   % electron negative (\em is taken)
\def\ep         {{\ensuremath{\Pe^+}}\xspace}
\def\epm        {{\ensuremath{\Pe^\pm}}\xspace} 
\def\epem       {{\ensuremath{\Pe^+\Pe^-}}\xspace}
%%%\def\ee         {\ensuremath{\Pe^-\Pe^-}\xspace}

\def\muon       {{\ensuremath{\Pmu}}\xspace}
\def\mup        {{\ensuremath{\Pmu^+}}\xspace}
\def\mun        {{\ensuremath{\Pmu^-}}\xspace} % muon negative (\mum is taken)
\def\mumu       {{\ensuremath{\Pmu^+\Pmu^-}}\xspace}

\def\tauon      {{\ensuremath{\Ptau}}\xspace}
\def\taup       {{\ensuremath{\Ptau^+}}\xspace}
\def\taum       {{\ensuremath{\Ptau^-}}\xspace}
\def\tautau     {{\ensuremath{\Ptau^+\Ptau^-}}\xspace}

\def\lepton     {{\ensuremath{\ell}}\xspace}
\def\ellm       {{\ensuremath{\ell^-}}\xspace}
\def\ellp       {{\ensuremath{\ell^+}}\xspace}
%%%\def\ellell     {\ensuremath{\ell^+ \ell^-}\xspace}

\def\neu        {{\ensuremath{\Pnu}}\xspace}
\def\neub       {{\ensuremath{\overline{\Pnu}}}\xspace}
%%%\def\nuenueb    {\ensuremath{\neu\neub}\xspace}
\def\neue       {{\ensuremath{\neu_e}}\xspace}
\def\neueb      {{\ensuremath{\neub_e}}\xspace}
%%%\def\neueneueb  {\ensuremath{\neue\neueb}\xspace}
\def\neum       {{\ensuremath{\neu_\mu}}\xspace}
\def\neumb      {{\ensuremath{\neub_\mu}}\xspace}
%%%\def\neumneumb  {\ensuremath{\neum\neumb}\xspace}
\def\neut       {{\ensuremath{\neu_\tau}}\xspace}
\def\neutb      {{\ensuremath{\neub_\tau}}\xspace}
%%%\def\neutneutb  {\ensuremath{\neut\neutb}\xspace}
\def\neul       {{\ensuremath{\neu_\ell}}\xspace}
\def\neulb      {{\ensuremath{\neub_\ell}}\xspace}
%%%\def\neulneulb  {\ensuremath{\neul\neulb}\xspace}

%% Gauge bosons and scalars

\def\g      {{\ensuremath{\Pgamma}}\xspace}
\def\H      {{\ensuremath{\PH^0}}\xspace}
\def\Hp     {{\ensuremath{\PH^+}}\xspace}
\def\Hm     {{\ensuremath{\PH^-}}\xspace}
\def\Hpm    {{\ensuremath{\PH^\pm}}\xspace}
\def\W      {{\ensuremath{\PW}}\xspace}
\def\Wp     {{\ensuremath{\PW^+}}\xspace}
\def\Wm     {{\ensuremath{\PW^-}}\xspace}
\def\Wpm    {{\ensuremath{\PW^\pm}}\xspace}
\def\Z      {{\ensuremath{\PZ}}\xspace}

%% Quarks

\def\quark     {{\ensuremath{\Pq}}\xspace}
\def\quarkbar  {{\ensuremath{\overline \quark}}\xspace}
\def\qqbar     {{\ensuremath{\quark\quarkbar}}\xspace}
\def\uquark    {{\ensuremath{\Pu}}\xspace}
\def\uquarkbar {{\ensuremath{\overline \uquark}}\xspace}
\def\uubar     {{\ensuremath{\uquark\uquarkbar}}\xspace}
\def\dquark    {{\ensuremath{\Pd}}\xspace}
\def\dquarkbar {{\ensuremath{\overline \dquark}}\xspace}
\def\ddbar     {{\ensuremath{\dquark\dquarkbar}}\xspace}
\def\squark    {{\ensuremath{\Ps}}\xspace}
\def\squarkbar {{\ensuremath{\overline \squark}}\xspace}
\def\ssbar     {{\ensuremath{\squark\squarkbar}}\xspace}
\def\cquark    {{\ensuremath{\Pc}}\xspace}
\def\cquarkbar {{\ensuremath{\overline \cquark}}\xspace}
\def\ccbar     {{\ensuremath{\cquark\cquarkbar}}\xspace}
\def\bquark    {{\ensuremath{\Pb}}\xspace}
\def\bquarkbar {{\ensuremath{\overline \bquark}}\xspace}
\def\bbbar     {{\ensuremath{\bquark\bquarkbar}}\xspace}
\def\tquark    {{\ensuremath{\Pt}}\xspace}
\def\tquarkbar {{\ensuremath{\overline \tquark}}\xspace}
\def\ttbar     {{\ensuremath{\tquark\tquarkbar}}\xspace}

%% Light mesons

\def\hadron {{\ensuremath{\Ph}}\xspace}
\def\pion   {{\ensuremath{\Ppi}}\xspace}
\def\piz    {{\ensuremath{\pion^0}}\xspace}
\def\pizs   {{\ensuremath{\pion^0\mbox\,\mathrm{s}}}\xspace}
\def\pip    {{\ensuremath{\pion^+}}\xspace}
\def\pim    {{\ensuremath{\pion^-}}\xspace}
\def\pipm   {{\ensuremath{\pion^\pm}}\xspace}
\def\pimp   {{\ensuremath{\pion^\mp}}\xspace}

\def\rhomeson {{\ensuremath{\Prho}}\xspace}
\def\rhoz     {{\ensuremath{\rhomeson^0}}\xspace}
\def\rhop     {{\ensuremath{\rhomeson^+}}\xspace}
\def\rhom     {{\ensuremath{\rhomeson^-}}\xspace}
\def\rhopm    {{\ensuremath{\rhomeson^\pm}}\xspace}
\def\rhomp    {{\ensuremath{\rhomeson^\mp}}\xspace}

\def\kaon    {{\ensuremath{\PK}}\xspace}
%%% do NOT use ensuremath here
  \def\Kbar    {{\kern 0.2em\overline{\kern -0.2em \PK}{}}\xspace}
\def\Kb      {{\ensuremath{\Kbar}}\xspace}
\def\KorKbar    {\kern 0.18em\optbar{\kern -0.18em K}{}\xspace}
\def\Kz      {{\ensuremath{\kaon^0}}\xspace}
\def\Kzb     {{\ensuremath{\Kbar{}^0}}\xspace}
\def\Kp      {{\ensuremath{\kaon^+}}\xspace}
\def\Km      {{\ensuremath{\kaon^-}}\xspace}
\def\Kpm     {{\ensuremath{\kaon^\pm}}\xspace}
\def\Kmp     {{\ensuremath{\kaon^\mp}}\xspace}
\def\KS      {{\ensuremath{\kaon^0_{\mathrm{ \scriptscriptstyle S}}}}\xspace}
\def\KL      {{\ensuremath{\kaon^0_{\mathrm{ \scriptscriptstyle L}}}}\xspace}
\def\Kstarz  {{\ensuremath{\kaon^{*0}}}\xspace}
\def\Kstarzb {{\ensuremath{\Kbar{}^{*0}}}\xspace}
\def\Kstar   {{\ensuremath{\kaon^*}}\xspace}
\def\Kstarb  {{\ensuremath{\Kbar{}^*}}\xspace}
\def\Kstarp  {{\ensuremath{\kaon^{*+}}}\xspace}
\def\Kstarm  {{\ensuremath{\kaon^{*-}}}\xspace}
\def\Kstarpm {{\ensuremath{\kaon^{*\pm}}}\xspace}
\def\Kstarmp {{\ensuremath{\kaon^{*\mp}}}\xspace}

\newcommand{\etaz}{\ensuremath{\Peta}\xspace}
\newcommand{\etapr}{\ensuremath{\Peta^{\prime}}\xspace}
\newcommand{\phiz}{\ensuremath{\Pphi}\xspace}
\newcommand{\omegaz}{\ensuremath{\Pomega}\xspace}

%% Heavy mesons

%%% do NOT use ensuremath here
  \def\Dbar    {{\kern 0.2em\overline{\kern -0.2em \PD}{}}\xspace}
\def\D       {{\ensuremath{\PD}}\xspace}
\def\Db      {{\ensuremath{\Dbar}}\xspace}
\def\DorDbar    {\kern 0.18em\optbar{\kern -0.18em D}{}\xspace}
\def\Dz      {{\ensuremath{\D^0}}\xspace}
\def\Dzb     {{\ensuremath{\Dbar{}^0}}\xspace}
\def\Dp      {{\ensuremath{\D^+}}\xspace}
\def\Dm      {{\ensuremath{\D^-}}\xspace}
\def\Dpm     {{\ensuremath{\D^\pm}}\xspace}
\def\Dmp     {{\ensuremath{\D^\mp}}\xspace}
\def\Dstar   {{\ensuremath{\D^*}}\xspace}
\def\Dstarb  {{\ensuremath{\Dbar{}^*}}\xspace}
\def\Dstarz  {{\ensuremath{\D^{*0}}}\xspace}
\def\Dstarzb {{\ensuremath{\Dbar{}^{*0}}}\xspace}
\def\Dstarp  {{\ensuremath{\D^{*+}}}\xspace}
\def\Dstarm  {{\ensuremath{\D^{*-}}}\xspace}
\def\Dstarpm {{\ensuremath{\D^{*\pm}}}\xspace}
\def\Dstarmp {{\ensuremath{\D^{*\mp}}}\xspace}
\def\Ds      {{\ensuremath{\D^+_\squark}}\xspace}
\def\Dsp     {{\ensuremath{\D^+_\squark}}\xspace}
\def\Dsm     {{\ensuremath{\D^-_\squark}}\xspace}
\def\Dspm    {{\ensuremath{\D^{\pm}_\squark}}\xspace}
\def\Dsmp    {{\ensuremath{\D^{\mp}_\squark}}\xspace}
\def\Dss     {{\ensuremath{\D^{*+}_\squark}}\xspace}
\def\Dssp    {{\ensuremath{\D^{*+}_\squark}}\xspace}
\def\Dssm    {{\ensuremath{\D^{*-}_\squark}}\xspace}
\def\Dsspm   {{\ensuremath{\D^{*\pm}_\squark}}\xspace}
\def\Dssmp   {{\ensuremath{\D^{*\mp}_\squark}}\xspace}

\def\B       {{\ensuremath{\PB}}\xspace}
%%% do NOT use ensuremath here
\def\Bbar    {{\ensuremath{\kern 0.18em\overline{\kern -0.18em \PB}{}}}\xspace}
\def\Bb      {{\ensuremath{\Bbar}}\xspace}
\def\BorBbar    {\kern 0.18em\optbar{\kern -0.18em B}{}\xspace}
\def\Bz      {{\ensuremath{\B^0}}\xspace}
\def\Bzb     {{\ensuremath{\Bbar{}^0}}\xspace}
\def\Bu      {{\ensuremath{\B^+}}\xspace}
\def\Bub     {{\ensuremath{\B^-}}\xspace}
\def\Bp      {{\ensuremath{\Bu}}\xspace}
\def\Bm      {{\ensuremath{\Bub}}\xspace}
\def\Bpm     {{\ensuremath{\B^\pm}}\xspace}
\def\Bmp     {{\ensuremath{\B^\mp}}\xspace}
\def\Bd      {{\ensuremath{\B^0}}\xspace}
\def\Bs      {{\ensuremath{\B^0_\squark}}\xspace}
\def\Bsb     {{\ensuremath{\Bbar{}^0_\squark}}\xspace}
\def\Bdb     {{\ensuremath{\Bbar{}^0}}\xspace}
\def\Bc      {{\ensuremath{\B_\cquark^+}}\xspace}
\def\Bcp     {{\ensuremath{\B_\cquark^+}}\xspace}
\def\Bcm     {{\ensuremath{\B_\cquark^-}}\xspace}
\def\Bcpm    {{\ensuremath{\B_\cquark^\pm}}\xspace}

%% Onia

\def\jpsi     {{\ensuremath{{\PJ\mskip -3mu/\mskip -2mu\Ppsi\mskip 2mu}}}\xspace}
\def\psitwos  {{\ensuremath{\Ppsi{(2S)}}}\xspace}
\def\psiprpr  {{\ensuremath{\Ppsi(3770)}}\xspace}
\def\etac     {{\ensuremath{\Peta_\cquark}}\xspace}
\def\chiczero {{\ensuremath{\Pchi_{\cquark 0}}}\xspace}
\def\chicone  {{\ensuremath{\Pchi_{\cquark 1}}}\xspace}
\def\chictwo  {{\ensuremath{\Pchi_{\cquark 2}}}\xspace}
  %\mathchardef\Upsilon="7107
  \def\Y#1S{\ensuremath{\PUpsilon{(#1S)}}\xspace}% no space before {...}!
\def\OneS  {{\Y1S}}
\def\TwoS  {{\Y2S}}
\def\ThreeS{{\Y3S}}
\def\FourS {{\Y4S}}
\def\FiveS {{\Y5S}}

\def\chic  {{\ensuremath{\Pchi_{c}}}\xspace}

%% Baryons

\def\proton      {{\ensuremath{\Pp}}\xspace}
\def\antiproton  {{\ensuremath{\overline \proton}}\xspace}
\def\neutron     {{\ensuremath{\Pn}}\xspace}
\def\antineutron {{\ensuremath{\overline \neutron}}\xspace}
\def\Deltares    {{\ensuremath{\PDelta}}\xspace}
\def\Deltaresbar {{\ensuremath{\overline \Deltares}}\xspace}
\def\Xires       {{\ensuremath{\PXi}}\xspace}
\def\Xiresbar    {{\ensuremath{\overline \Xires}}\xspace}
\def\Lz          {{\ensuremath{\PLambda}}\xspace}
\def\Lbar        {{\ensuremath{\kern 0.1em\overline{\kern -0.1em\PLambda}}}\xspace}
\def\LorLbar    {\kern 0.18em\optbar{\kern -0.18em \PLambda}{}\xspace}
\def\Lambdares   {{\ensuremath{\PLambda}}\xspace}
\def\Lambdaresbar{{\ensuremath{\Lbar}}\xspace}
\def\Sigmares    {{\ensuremath{\PSigma}}\xspace}
\def\Sigmaresbar {{\ensuremath{\overline \Sigmares}}\xspace}
\def\Omegares    {{\ensuremath{\POmega}}\xspace}
\def\Omegaresbar {{\ensuremath{\overline \POmega}}\xspace}

%%% do NOT use ensuremath here
 % \def\Deltabar{\kern 0.25em\overline{\kern -0.25em \Deltares}{}\xspace}
 % \def\Sigbar{\kern 0.2em\overline{\kern -0.2em \Sigma}{}\xspace}
 % \def\Xibar{\kern 0.2em\overline{\kern -0.2em \Xi}{}\xspace}
 % \def\Obar{\kern 0.2em\overline{\kern -0.2em \Omega}{}\xspace}
 % \def\Nbar{\kern 0.2em\overline{\kern -0.2em N}{}\xspace}
 % \def\Xb{\kern 0.2em\overline{\kern -0.2em X}{}\xspace}

\def\Lb      {{\ensuremath{\Lz^0_\bquark}}\xspace}
\def\Lbbar   {{\ensuremath{\Lbar{}^0_\bquark}}\xspace}
\def\Lc      {{\ensuremath{\Lz^+_\cquark}}\xspace}
\def\Lcbar   {{\ensuremath{\Lbar{}^-_\cquark}}\xspace}
\def\Xib     {{\ensuremath{\Xires_\bquark}}\xspace}
\def\Xibz    {{\ensuremath{\Xires^0_\bquark}}\xspace}
\def\Xibm    {{\ensuremath{\Xires^-_\bquark}}\xspace}
\def\Xibbar  {{\ensuremath{\Xiresbar{}_\bquark}}\xspace}
\def\Xibbarz {{\ensuremath{\Xiresbar{}_\bquark^0}}\xspace}
\def\Xibbarp {{\ensuremath{\Xiresbar{}_\bquark^+}}\xspace}
\def\Xic     {{\ensuremath{\Xires_\cquark}}\xspace}
\def\Xicz    {{\ensuremath{\Xires^0_\cquark}}\xspace}
\def\Xicp    {{\ensuremath{\Xires^+_\cquark}}\xspace}
\def\Xicbar  {{\ensuremath{\Xiresbar{}_\cquark}}\xspace}
\def\Xicbarz {{\ensuremath{\Xiresbar{}_\cquark^0}}\xspace}
\def\Xicbarm {{\ensuremath{\Xiresbar{}_\cquark^-}}\xspace}
\def\Omegac    {{\ensuremath{\Omegares^0_\cquark}}\xspace}
\def\Omegacbar {{\ensuremath{\Omegaresbar{}_\cquark^0}}\xspace}
\def\Omegab    {{\ensuremath{\Omegares^-_\bquark}}\xspace}
\def\Omegabbar {{\ensuremath{\Omegaresbar{}_\bquark^+}}\xspace}

%%%%%%%%%%%%%%%%%%
% Physics symbols
%%%%%%%%%%%%%%%%%

%% Decays
\def\BF         {{\ensuremath{\mathcal{B}}}\xspace}
\def\BRvis      {{\ensuremath{\BR_{\mathrm{{vis}}}}}}
\def\BR         {\BF}
\newcommand{\decay}[2]{\ensuremath{#1\!\to #2}\xspace}         % {\Pa}{\Pb \Pc}
\def\ra                 {\ensuremath{\rightarrow}\xspace}
\def\to                 {\ensuremath{\rightarrow}\xspace}

%% Lifetimes
\newcommand{\tauBs}{{\ensuremath{\tau_{\Bs}}}\xspace}
\newcommand{\tauBd}{{\ensuremath{\tau_{\Bd}}}\xspace}
\newcommand{\tauBz}{{\ensuremath{\tau_{\Bz}}}\xspace}
\newcommand{\tauBu}{{\ensuremath{\tau_{\Bp}}}\xspace}
\newcommand{\tauDp}{{\ensuremath{\tau_{\Dp}}}\xspace}
\newcommand{\tauDz}{{\ensuremath{\tau_{\Dz}}}\xspace}
\newcommand{\tauL}{{\ensuremath{\tau_{\mathrm{ L}}}}\xspace}
\newcommand{\tauH}{{\ensuremath{\tau_{\mathrm{ H}}}}\xspace}

%% Masses
\newcommand{\mBd}{{\ensuremath{m_{\Bd}}}\xspace}
\newcommand{\mBp}{{\ensuremath{m_{\Bp}}}\xspace}
\newcommand{\mBs}{{\ensuremath{m_{\Bs}}}\xspace}
\newcommand{\mBc}{{\ensuremath{m_{\Bc}}}\xspace}
\newcommand{\mLb}{{\ensuremath{m_{\Lb}}}\xspace}

%% EW theory, groups
\def\grpsuthree {{\ensuremath{\mathrm{SU}(3)}}\xspace}
\def\grpsutw    {{\ensuremath{\mathrm{SU}(2)}}\xspace}
\def\grpuone    {{\ensuremath{\mathrm{U}(1)}}\xspace}

\def\ssqtw   {{\ensuremath{\sin^{2}\!\theta_{\mathrm{W}}}}\xspace}
\def\csqtw   {{\ensuremath{\cos^{2}\!\theta_{\mathrm{W}}}}\xspace}
\def\stw     {{\ensuremath{\sin\theta_{\mathrm{W}}}}\xspace}
\def\ctw     {{\ensuremath{\cos\theta_{\mathrm{W}}}}\xspace}
\def\ssqtwef {{\ensuremath{{\sin}^{2}\theta_{\mathrm{W}}^{\mathrm{eff}}}}\xspace}
\def\csqtwef {{\ensuremath{{\cos}^{2}\theta_{\mathrm{W}}^{\mathrm{eff}}}}\xspace}
\def\stwef   {{\ensuremath{\sin\theta_{\mathrm{W}}^{\mathrm{eff}}}}\xspace}
\def\ctwef   {{\ensuremath{\cos\theta_{\mathrm{W}}^{\mathrm{eff}}}}\xspace}
\def\gv      {{\ensuremath{g_{\mbox{\tiny V}}}}\xspace}
\def\ga      {{\ensuremath{g_{\mbox{\tiny A}}}}\xspace}

\def\order   {{\ensuremath{\mathcal{O}}}\xspace}
\def\ordalph {{\ensuremath{\mathcal{O}(\alpha)}}\xspace}
\def\ordalsq {{\ensuremath{\mathcal{O}(\alpha^{2})}}\xspace}
\def\ordalcb {{\ensuremath{\mathcal{O}(\alpha^{3})}}\xspace}

%% QCD parameters
\newcommand{\as}{{\ensuremath{\alpha_s}}\xspace}
\newcommand{\MSb}{{\ensuremath{\overline{\mathrm{MS}}}}\xspace}
\newcommand{\lqcd}{{\ensuremath{\Lambda_{\mathrm{QCD}}}}\xspace}
\def\qsq       {{\ensuremath{q^2}}\xspace}

%% CKM, CP violation

\def\eps   {{\ensuremath{\varepsilon}}\xspace}
\def\epsK  {{\ensuremath{\varepsilon_K}}\xspace}
\def\epsB  {{\ensuremath{\varepsilon_B}}\xspace}
\def\epsp  {{\ensuremath{\varepsilon^\prime_K}}\xspace}

\def\CP                {{\ensuremath{C\!P}}\xspace}
\def\CPT               {{\ensuremath{C\!PT}}\xspace}

\def\rhobar {{\ensuremath{\overline \rho}}\xspace}
\def\etabar {{\ensuremath{\overline \eta}}\xspace}

\def\Vud  {{\ensuremath{V_{\uquark\dquark}}}\xspace}
\def\Vcd  {{\ensuremath{V_{\cquark\dquark}}}\xspace}
\def\Vtd  {{\ensuremath{V_{\tquark\dquark}}}\xspace}
\def\Vus  {{\ensuremath{V_{\uquark\squark}}}\xspace}
\def\Vcs  {{\ensuremath{V_{\cquark\squark}}}\xspace}
\def\Vts  {{\ensuremath{V_{\tquark\squark}}}\xspace}
\def\Vub  {{\ensuremath{V_{\uquark\bquark}}}\xspace}
\def\Vcb  {{\ensuremath{V_{\cquark\bquark}}}\xspace}
\def\Vtb  {{\ensuremath{V_{\tquark\bquark}}}\xspace}
\def\Vuds  {{\ensuremath{V_{\uquark\dquark}^\ast}}\xspace}
\def\Vcds  {{\ensuremath{V_{\cquark\dquark}^\ast}}\xspace}
\def\Vtds  {{\ensuremath{V_{\tquark\dquark}^\ast}}\xspace}
\def\Vuss  {{\ensuremath{V_{\uquark\squark}^\ast}}\xspace}
\def\Vcss  {{\ensuremath{V_{\cquark\squark}^\ast}}\xspace}
\def\Vtss  {{\ensuremath{V_{\tquark\squark}^\ast}}\xspace}
\def\Vubs  {{\ensuremath{V_{\uquark\bquark}^\ast}}\xspace}
\def\Vcbs  {{\ensuremath{V_{\cquark\bquark}^\ast}}\xspace}
\def\Vtbs  {{\ensuremath{V_{\tquark\bquark}^\ast}}\xspace}

%% Oscillations

\newcommand{\dm}{{\ensuremath{\Delta m}}\xspace}
\newcommand{\dms}{{\ensuremath{\Delta m_{\squark}}}\xspace}
\newcommand{\dmd}{{\ensuremath{\Delta m_{\dquark}}}\xspace}
\newcommand{\DG}{{\ensuremath{\Delta\Gamma}}\xspace}
\newcommand{\DGs}{{\ensuremath{\Delta\Gamma_{\squark}}}\xspace}
\newcommand{\DGd}{{\ensuremath{\Delta\Gamma_{\dquark}}}\xspace}
\newcommand{\Gs}{{\ensuremath{\Gamma_{\squark}}}\xspace}
\newcommand{\Gd}{{\ensuremath{\Gamma_{\dquark}}}\xspace}
\newcommand{\MBq}{{\ensuremath{M_{\B_\quark}}}\xspace}
\newcommand{\DGq}{{\ensuremath{\Delta\Gamma_{\quark}}}\xspace}
\newcommand{\Gq}{{\ensuremath{\Gamma_{\quark}}}\xspace}
\newcommand{\dmq}{{\ensuremath{\Delta m_{\quark}}}\xspace}
\newcommand{\GL}{{\ensuremath{\Gamma_{\mathrm{ L}}}}\xspace}
\newcommand{\GH}{{\ensuremath{\Gamma_{\mathrm{ H}}}}\xspace}
\newcommand{\DGsGs}{{\ensuremath{\Delta\Gamma_{\squark}/\Gamma_{\squark}}}\xspace}
\newcommand{\Delm}{{\mbox{$\Delta m $}}\xspace}
\newcommand{\ACP}{{\ensuremath{{\mathcal{A}}^{\CP}}}\xspace}
\newcommand{\Adir}{{\ensuremath{{\mathcal{A}}^{\mathrm{ dir}}}}\xspace}
\newcommand{\Amix}{{\ensuremath{{\mathcal{A}}^{\mathrm{ mix}}}}\xspace}
\newcommand{\ADelta}{{\ensuremath{{\mathcal{A}}^\Delta}}\xspace}
\newcommand{\phid}{{\ensuremath{\phi_{\dquark}}}\xspace}
\newcommand{\sinphid}{{\ensuremath{\sin\!\phid}}\xspace}
\newcommand{\phis}{{\ensuremath{\phi_{\squark}}}\xspace}
\newcommand{\betas}{{\ensuremath{\beta_{\squark}}}\xspace}
\newcommand{\sbetas}{{\ensuremath{\sigma(\beta_{\squark})}}\xspace}
\newcommand{\stbetas}{{\ensuremath{\sigma(2\beta_{\squark})}}\xspace}
\newcommand{\stphis}{{\ensuremath{\sigma(\phi_{\squark})}}\xspace}
\newcommand{\sinphis}{{\ensuremath{\sin\!\phis}}\xspace}

%% Tagging
\newcommand{\edet}{{\ensuremath{\varepsilon_{\mathrm{ det}}}}\xspace}
\newcommand{\erec}{{\ensuremath{\varepsilon_{\mathrm{ rec/det}}}}\xspace}
\newcommand{\esel}{{\ensuremath{\varepsilon_{\mathrm{ sel/rec}}}}\xspace}
\newcommand{\etrg}{{\ensuremath{\varepsilon_{\mathrm{ trg/sel}}}}\xspace}
\newcommand{\etot}{{\ensuremath{\varepsilon_{\mathrm{ tot}}}}\xspace}

\newcommand{\mistag}{\ensuremath{\omega}\xspace}
\newcommand{\wcomb}{\ensuremath{\omega^{\mathrm{comb}}}\xspace}
\newcommand{\etag}{{\ensuremath{\varepsilon_{\mathrm{tag}}}}\xspace}
\newcommand{\etagcomb}{{\ensuremath{\varepsilon_{\mathrm{tag}}^{\mathrm{comb}}}}\xspace}
\newcommand{\effeff}{\ensuremath{\varepsilon_{\mathrm{eff}}}\xspace}
\newcommand{\effeffcomb}{\ensuremath{\varepsilon_{\mathrm{eff}}^{\mathrm{comb}}}\xspace}
\newcommand{\efftag}{{\ensuremath{\etag(1-2\omega)^2}}\xspace}
\newcommand{\effD}{{\ensuremath{\etag D^2}}\xspace}

\newcommand{\etagprompt}{{\ensuremath{\varepsilon_{\mathrm{ tag}}^{\mathrm{Pr}}}}\xspace}
\newcommand{\etagLL}{{\ensuremath{\varepsilon_{\mathrm{ tag}}^{\mathrm{LL}}}}\xspace}

%% Key decay channels

\def\BdToKstmm    {\decay{\Bd}{\Kstarz\mup\mun}}
\def\BdbToKstmm   {\decay{\Bdb}{\Kstarzb\mup\mun}}

\def\BsToJPsiPhi  {\decay{\Bs}{\jpsi\phi}}
\def\BdToJPsiKst  {\decay{\Bd}{\jpsi\Kstarz}}
\def\BdbToJPsiKst {\decay{\Bdb}{\jpsi\Kstarzb}}

\def\BsPhiGam     {\decay{\Bs}{\phi \g}}
\def\BdKstGam     {\decay{\Bd}{\Kstarz \g}}

\def\BTohh        {\decay{\B}{\Ph^+ \Ph'^-}}
\def\BdTopipi     {\decay{\Bd}{\pip\pim}}
\def\BdToKpi      {\decay{\Bd}{\Kp\pim}}
\def\BsToKK       {\decay{\Bs}{\Kp\Km}}
\def\BsTopiK      {\decay{\Bs}{\pip\Km}}

%% Rare decays
\def\BdKstee  {\decay{\Bd}{\Kstarz\epem}}
\def\BdbKstee {\decay{\Bdb}{\Kstarzb\epem}}
\def\bsll     {\decay{\bquark}{\squark \ell^+ \ell^-}}
\def\AFB      {\ensuremath{A_{\mathrm{FB}}}\xspace}
\def\FL       {\ensuremath{F_{\mathrm{L}}}\xspace}
\def\AT#1     {\ensuremath{A_{\mathrm{T}}^{#1}}\xspace}           % 2
\def\btosgam  {\decay{\bquark}{\squark \g}}
\def\btodgam  {\decay{\bquark}{\dquark \g}}
\def\Bsmm     {\decay{\Bs}{\mup\mun}}
\def\Bdmm     {\decay{\Bd}{\mup\mun}}
\def\ctl       {\ensuremath{\cos{\theta_\ell}}\xspace}
\def\ctk       {\ensuremath{\cos{\theta_K}}\xspace}

%% Wilson coefficients and operators
\def\C#1      {\ensuremath{\mathcal{C}_{#1}}\xspace}                       % 9
\def\Cp#1     {\ensuremath{\mathcal{C}_{#1}^{'}}\xspace}                    % 7
\def\Ceff#1   {\ensuremath{\mathcal{C}_{#1}^{\mathrm{(eff)}}}\xspace}        % 9  
\def\Cpeff#1  {\ensuremath{\mathcal{C}_{#1}^{'\mathrm{(eff)}}}\xspace}       % 7
\def\Ope#1    {\ensuremath{\mathcal{O}_{#1}}\xspace}                       % 2
\def\Opep#1   {\ensuremath{\mathcal{O}_{#1}^{'}}\xspace}                    % 7

%% Charm

\def\xprime     {\ensuremath{x^{\prime}}\xspace}
\def\yprime     {\ensuremath{y^{\prime}}\xspace}
\def\ycp        {\ensuremath{y_{\CP}}\xspace}
\def\agamma     {\ensuremath{A_{\Gamma}}\xspace}
%%%\def\kpi        {\ensuremath{\PK\Ppi}\xspace}
%%%\def\kk         {\ensuremath{\PK\PK}\xspace}
%%%\def\dkpi       {\decay{\PD}{\PK\Ppi}}
%%%\def\dkk        {\decay{\PD}{\PK\PK}}
\def\dkpicf     {\decay{\Dz}{\Km\pip}}

%% QM
\newcommand{\bra}[1]{\ensuremath{\langle #1|}}             % {a}
\newcommand{\ket}[1]{\ensuremath{|#1\rangle}}              % {b}
\newcommand{\braket}[2]{\ensuremath{\langle #1|#2\rangle}} % {a}{b}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Units
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\unit}[1]{\ensuremath{\mathrm{ \,#1}}\xspace}          % {kg}

%% Energy and momentum
\newcommand{\tev}{\ifthenelse{\boolean{inbibliography}}{\ensuremath{~T\kern -0.05em eV}\xspace}{\ensuremath{\mathrm{\,Te\kern -0.1em V}}}\xspace}
\newcommand{\gev}{\ensuremath{\mathrm{\,Ge\kern -0.1em V}}\xspace}
\newcommand{\mev}{\ensuremath{\mathrm{\,Me\kern -0.1em V}}\xspace}
\newcommand{\kev}{\ensuremath{\mathrm{\,ke\kern -0.1em V}}\xspace}
\newcommand{\ev}{\ensuremath{\mathrm{\,e\kern -0.1em V}}\xspace}
\newcommand{\gevc}{\ensuremath{{\mathrm{\,Ge\kern -0.1em V\!/}c}}\xspace}
\newcommand{\mevc}{\ensuremath{{\mathrm{\,Me\kern -0.1em V\!/}c}}\xspace}
\newcommand{\gevcc}{\ensuremath{{\mathrm{\,Ge\kern -0.1em V\!/}c^2}}\xspace}
\newcommand{\gevgevcccc}{\ensuremath{{\mathrm{\,Ge\kern -0.1em V^2\!/}c^4}}\xspace}
\newcommand{\mevcc}{\ensuremath{{\mathrm{\,Me\kern -0.1em V\!/}c^2}}\xspace}

%% Distance and area
\def\km   {\ensuremath{\mathrm{ \,km}}\xspace}
\def\m    {\ensuremath{\mathrm{ \,m}}\xspace}
\def\ma   {\ensuremath{{\mathrm{ \,m}}^2}\xspace}
\def\cm   {\ensuremath{\mathrm{ \,cm}}\xspace}
\def\cma  {\ensuremath{{\mathrm{ \,cm}}^2}\xspace}
\def\mm   {\ensuremath{\mathrm{ \,mm}}\xspace}
\def\mma  {\ensuremath{{\mathrm{ \,mm}}^2}\xspace}
\def\mum  {\ensuremath{{\,\upmu\mathrm{m}}}\xspace}
\def\muma {\ensuremath{{\,\upmu\mathrm{m}^2}}\xspace}
\def\nm   {\ensuremath{\mathrm{ \,nm}}\xspace}
\def\fm   {\ensuremath{\mathrm{ \,fm}}\xspace}
\def\barn{\ensuremath{\mathrm{ \,b}}\xspace}
%%%\def\barnhyph{\ensuremath{\mathrm{ -b}}\xspace}
\def\mbarn{\ensuremath{\mathrm{ \,mb}}\xspace}
\def\mub{\ensuremath{{\mathrm{ \,\upmu b}}}\xspace}
%%%\def\mbarnhyph{\ensuremath{\mathrm{ -mb}}\xspace}
\def\nb {\ensuremath{\mathrm{ \,nb}}\xspace}
\def\invnb {\ensuremath{\mbox{\,nb}^{-1}}\xspace}
\def\pb {\ensuremath{\mathrm{ \,pb}}\xspace}
\def\invpb {\ensuremath{\mbox{\,pb}^{-1}}\xspace}
\def\fb   {\ensuremath{\mbox{\,fb}}\xspace}
\def\invfb   {\ensuremath{\mbox{\,fb}^{-1}}\xspace}
\def\ab   {\ensuremath{\mbox{\,ab}}\xspace}
\def\invab   {\ensuremath{\mbox{\,ab}^{-1}}\xspace}

%% Time 
\def\sec  {\ensuremath{\mathrm{{\,s}}}\xspace}
\def\ms   {\ensuremath{{\mathrm{ \,ms}}}\xspace}
\def\mus  {\ensuremath{{\,\upmu{\mathrm{ s}}}}\xspace}
\def\ns   {\ensuremath{{\mathrm{ \,ns}}}\xspace}
\def\ps   {\ensuremath{{\mathrm{ \,ps}}}\xspace}
\def\fs   {\ensuremath{\mathrm{ \,fs}}\xspace}

\def\mhz  {\ensuremath{{\mathrm{ \,MHz}}}\xspace}
\def\khz  {\ensuremath{{\mathrm{ \,kHz}}}\xspace}
\def\hz   {\ensuremath{{\mathrm{ \,Hz}}}\xspace}

\def\invps{\ensuremath{{\mathrm{ \,ps^{-1}}}}\xspace}
\def\invns{\ensuremath{{\mathrm{ \,ns^{-1}}}}\xspace}

\def\yr   {\ensuremath{\mathrm{ \,yr}}\xspace}
\def\hr   {\ensuremath{\mathrm{ \,hr}}\xspace}

%% Temperature
\def\degc {\ensuremath{^\circ}{C}\xspace}
\def\degk {\ensuremath {\mathrm{ K}}\xspace}

%% Material lengths, radiation
\def\Xrad {\ensuremath{X_0}\xspace}
\def\NIL{\ensuremath{\lambda_{int}}\xspace}
\def\mip {MIP\xspace}
\def\neutroneq {\ensuremath{\mathrm{ \,n_{eq}}}\xspace}
\def\neqcmcm {\ensuremath{\mathrm{ \,n_{eq} / cm^2}}\xspace}
\def\kRad {\ensuremath{\mathrm{ \,kRad}}\xspace}
\def\MRad {\ensuremath{\mathrm{ \,MRad}}\xspace}
\def\ci {\ensuremath{\mathrm{ \,Ci}}\xspace}
\def\mci {\ensuremath{\mathrm{ \,mCi}}\xspace}

%% Uncertainties
\def\sx    {\ensuremath{\sigma_x}\xspace}    
\def\sy    {\ensuremath{\sigma_y}\xspace}   
\def\sz    {\ensuremath{\sigma_z}\xspace}    

\newcommand{\stat}{\ensuremath{\mathrm{\,(stat)}}\xspace}
\newcommand{\syst}{\ensuremath{\mathrm{\,(syst)}}\xspace}

%% Maths

\def\order{{\ensuremath{\mathcal{O}}}\xspace}
\newcommand{\chisq}{\ensuremath{\chi^2}\xspace}
\newcommand{\chisqndf}{\ensuremath{\chi^2/\mathrm{ndf}}\xspace}
\newcommand{\chisqip}{\ensuremath{\chi^2_{\text{IP}}}\xspace}
\newcommand{\chisqvs}{\ensuremath{\chi^2_{\text{VS}}}\xspace}
\newcommand{\chisqvtx}{\ensuremath{\chi^2_{\text{vtx}}}\xspace}
\newcommand{\chisqvtxndf}{\ensuremath{\chi^2_{\text{vtx}}/\mathrm{ndf}}\xspace}

\def\deriv {\ensuremath{\mathrm{d}}}

\def\gsim{{~\raise.15em\hbox{$>$}\kern-.85em
          \lower.35em\hbox{$\sim$}~}\xspace}
\def\lsim{{~\raise.15em\hbox{$<$}\kern-.85em
          \lower.35em\hbox{$\sim$}~}\xspace}

\newcommand{\mean}[1]{\ensuremath{\left\langle #1 \right\rangle}} % {x}
\newcommand{\abs}[1]{\ensuremath{\left\|#1\right\|}} % {x}
\newcommand{\Real}{\ensuremath{\mathcal{R}e}\xspace}
\newcommand{\Imag}{\ensuremath{\mathcal{I}m}\xspace}

\def\PDF {PDF\xspace}

\def\sPlot{\mbox{\em sPlot}\xspace}
%%%\def\sWeight{\mbox{\em sWeight}\xspace}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Kinematics
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%% Energy, Momenta
\def\Ebeam {\ensuremath{E_{\mbox{\tiny BEAM}}}\xspace}
\def\sqs   {\ensuremath{\protect\sqrt{s}}\xspace}

\def\ptot       {\mbox{$p$}\xspace}
\def\pt         {\mbox{$p_{\mathrm{ T}}$}\xspace}
\def\et         {\mbox{$E_{\mathrm{ T}}$}\xspace}
\def\mt         {\mbox{$M_{\mathrm{ T}}$}\xspace}
\def\dpp        {\ensuremath{\Delta p/p}\xspace}
\def\msq        {\ensuremath{m^2}\xspace}
\newcommand{\dedx}{\ensuremath{\mathrm{d}\hspace{-0.1em}E/\mathrm{d}x}\xspace}

%% PID

\def\dllkpi     {\ensuremath{\mathrm{DLL}_{\kaon\pion}}\xspace}
\def\dllppi     {\ensuremath{\mathrm{DLL}_{\proton\pion}}\xspace}
\def\dllepi     {\ensuremath{\mathrm{DLL}_{\electron\pion}}\xspace}
\def\dllmupi    {\ensuremath{\mathrm{DLL}_{\muon\pi}}\xspace}

%% Geometry
%%%\def\mphi       {\mbox{$\phi$}\xspace}
%%%\def\mtheta     {\mbox{$\theta$}\xspace}
%%%\def\ctheta     {\mbox{$\cos\theta$}\xspace}
%%%\def\stheta     {\mbox{$\sin\theta$}\xspace}
%%%\def\ttheta     {\mbox{$\tan\theta$}\xspace}

\def\degrees{\ensuremath{^{\circ}}\xspace}
\def\krad {\ensuremath{\mathrm{ \,krad}}\xspace}
\def\mrad{\ensuremath{\mathrm{ \,mrad}}\xspace}
\def\rad{\ensuremath{\mathrm{ \,rad}}\xspace}

%% Accelerator
\def\betastar {\ensuremath{\beta^*}}
\newcommand{\lum} {\ensuremath{\mathcal{L}}\xspace}
\newcommand{\intlum}[1]{\ensuremath{\int\lum=#1}\xspace}  % {2 \,\invfb}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Software
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%% Programs
%%%\def\ansys      {\mbox{\textsc{Ansys}}\xspace}
\def\bcvegpy    {\mbox{\textsc{Bcvegpy}}\xspace}
\def\boole      {\mbox{\textsc{Boole}}\xspace}
\def\brunel     {\mbox{\textsc{Brunel}}\xspace}
\def\davinci    {\mbox{\textsc{DaVinci}}\xspace}
\def\dirac      {\mbox{\textsc{Dirac}}\xspace}
%%%\def\erasmus    {\mbox{\textsc{Erasmus}}\xspace}
\def\evtgen     {\mbox{\textsc{EvtGen}}\xspace}
\def\fewz       {\mbox{\textsc{Fewz}}\xspace}
\def\fluka      {\mbox{\textsc{Fluka}}\xspace}
\def\ganga      {\mbox{\textsc{Ganga}}\xspace}
%%%\def\garfield   {\mbox{\textsc{Garfield}}\xspace}
\def\gaudi      {\mbox{\textsc{Gaudi}}\xspace}
\def\gauss      {\mbox{\textsc{Gauss}}\xspace}
\def\geant      {\mbox{\textsc{Geant4}}\xspace}
\def\hepmc      {\mbox{\textsc{HepMC}}\xspace}
\def\herwig     {\mbox{\textsc{Herwig}}\xspace}
\def\moore      {\mbox{\textsc{Moore}}\xspace}
\def\neurobayes {\mbox{\textsc{NeuroBayes}}\xspace}
\def\photos     {\mbox{\textsc{Photos}}\xspace}
\def\powheg     {\mbox{\textsc{Powheg}}\xspace}
%%%\def\pyroot     {\mbox{\textsc{PyRoot}}\xspace}
\def\pythia     {\mbox{\textsc{Pythia}}\xspace}
\def\resbos     {\mbox{\textsc{ResBos}}\xspace}
\def\roofit     {\mbox{\textsc{RooFit}}\xspace}
\def\root       {\mbox{\textsc{Root}}\xspace}
\def\spice      {\mbox{\textsc{Spice}}\xspace}
%%%\def\tosca      {\mbox{\textsc{Tosca}}\xspace}
\def\urania     {\mbox{\textsc{Urania}}\xspace}

%% Languages
\def\cpp        {\mbox{\textsc{C\raisebox{0.1em}{{\footnotesize{++}}}}}\xspace}
%%%\def\python     {\mbox{\textsc{Python}}\xspace}
\def\ruby       {\mbox{\textsc{Ruby}}\xspace}
\def\fortran    {\mbox{\textsc{Fortran}}\xspace}
\def\svn        {\mbox{\textsc{SVN}}\xspace}

%% Data processing
\def\kbytes     {\ensuremath{{\mathrm{ \,kbytes}}}\xspace}
\def\kbsps      {\ensuremath{{\mathrm{ \,kbytes/s}}}\xspace}
\def\kbits      {\ensuremath{{\mathrm{ \,kbits}}}\xspace}
\def\kbsps      {\ensuremath{{\mathrm{ \,kbits/s}}}\xspace}
\def\mbsps      {\ensuremath{{\mathrm{ \,Mbits/s}}}\xspace}
\def\mbytes     {\ensuremath{{\mathrm{ \,Mbytes}}}\xspace}
\def\mbps       {\ensuremath{{\mathrm{ \,Mbyte/s}}}\xspace}
\def\mbsps      {\ensuremath{{\mathrm{ \,Mbytes/s}}}\xspace}
\def\gbsps      {\ensuremath{{\mathrm{ \,Gbits/s}}}\xspace}
\def\gbytes     {\ensuremath{{\mathrm{ \,Gbytes}}}\xspace}
\def\gbsps      {\ensuremath{{\mathrm{ \,Gbytes/s}}}\xspace}
\def\tbytes     {\ensuremath{{\mathrm{ \,Tbytes}}}\xspace}
\def\tbpy       {\ensuremath{{\mathrm{ \,Tbytes/yr}}}\xspace}

\def\dst        {DST\xspace}

%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Detector related
%%%%%%%%%%%%%%%%%%%%%%%%%%%

%% Detector technologies
\def\nonn {\ensuremath{\mathrm{{ \mathit{n^+}} \mbox{-} on\mbox{-}{ \mathit{n}}}}\xspace}
\def\ponn {\ensuremath{\mathrm{{ \mathit{p^+}} \mbox{-} on\mbox{-}{ \mathit{n}}}}\xspace}
\def\nonp {\ensuremath{\mathrm{{ \mathit{n^+}} \mbox{-} on\mbox{-}{ \mathit{p}}}}\xspace}
\def\cvd  {CVD\xspace}
\def\mwpc {MWPC\xspace}
\def\gem  {GEM\xspace}

%% Detector components, electronics
\def\tell1  {TELL1\xspace}
\def\ukl1   {UKL1\xspace}
\def\beetle {Beetle\xspace}
\def\otis   {OTIS\xspace}
\def\croc   {CROC\xspace}
\def\carioca {CARIOCA\xspace}
\def\dialog {DIALOG\xspace}
\def\sync   {SYNC\xspace}
\def\cardiac {CARDIAC\xspace}
\def\gol    {GOL\xspace}
\def\vcsel  {VCSEL\xspace}
\def\ttc    {TTC\xspace}
\def\ttcrx  {TTCrx\xspace}
\def\hpd    {HPD\xspace}
\def\pmt    {PMT\xspace}
\def\specs  {SPECS\xspace}
\def\elmb   {ELMB\xspace}
\def\fpga   {FPGA\xspace}
\def\plc    {PLC\xspace}
\def\rasnik {RASNIK\xspace}
\def\elmb   {ELMB\xspace}
\def\can    {CAN\xspace}
\def\lvds   {LVDS\xspace}
\def\ntc    {NTC\xspace}
\def\adc    {ADC\xspace}
\def\led    {LED\xspace}
\def\ccd    {CCD\xspace}
\def\hv     {HV\xspace}
\def\lv     {LV\xspace}
\def\pvss   {PVSS\xspace}
\def\cmos   {CMOS\xspace}
\def\fifo   {FIFO\xspace}
\def\ccpc   {CCPC\xspace}

%% Chemical symbols
\def\cfourften     {\ensuremath{\mathrm{ C_4 F_{10}}}\xspace}
\def\cffour        {\ensuremath{\mathrm{ CF_4}}\xspace}
\def\cotwo         {\ensuremath{\mathrm{ CO_2}}\xspace} 
\def\csixffouteen  {\ensuremath{\mathrm{ C_6 F_{14}}}\xspace} 
\def\mgftwo     {\ensuremath{\mathrm{ Mg F_2}}\xspace} 
\def\siotwo     {\ensuremath{\mathrm{ SiO_2}}\xspace} 

%%%%%%%%%%%%%%%
% Special Text 
%%%%%%%%%%%%%%%
\newcommand{\eg}{\mbox{\itshape e.g.}\xspace}
\newcommand{\ie}{\mbox{\itshape i.e.}\xspace}
\newcommand{\etal}{\mbox{\itshape et al.}\xspace}
\newcommand{\etc}{\mbox{\itshape etc.}\xspace}
\newcommand{\cf}{\mbox{\itshape cf.}\xspace}
\newcommand{\ffp}{\mbox{\itshape ff.}\xspace}
\newcommand{\vs}{\mbox{\itshape vs.}\xspace}

